Continuous Herded Gibbs Sampling

Herding is a technique to sequentially generate deterministic samples from a probability distribution. In this work, we propose a continuous herded Gibbs sampler that combines kernel herding on continuous densities with the Gibbs sampling idea. Our algorithm allows for deterministically sampling from high-dimensional multivariate probability densities, without directly sampling from the joint density. Experiments with Gaussian mixture densities indicate that the L2 error decreases similarly to kernel herding, while the computation time is significantly lower, i.e., linear in the number of dimensions.

==> herding_error.tex <==
% This file was created by tikzplotlib v0.9.8.
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
label style={font=\footnotesize},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
legend style={font=\footnotesize},
tick align=outside,
tick label style={font=\footnotesize},
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={number of samples \(\displaystyle T\)},
xmin=-48.95, xmax=1049.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={inverse herding error \(\displaystyle 1/\mathcal{E}_T\)},
ymin=-1.15631972361787, ymax=29.8934170295597,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
1 0.255584002197235
2 0.367664901963735
3 0.458079354360284
4 0.537167169925932
5 0.609174448169477
6 0.675252671656887
7 0.737313614687354
8 0.795919387925952
9 0.851882658959698
10 0.905460430031493
11 0.957284083703022
12 1.00716926550376
13 1.055641291188
14 1.10377434454906
15 1.1507727322643
16 1.19703514321684
17 1.24231080445842
18 1.28727122694421
19 1.33213243729913
20 1.37581596163996
21 1.41881930719788
22 1.46227132664831
23 1.50395097247472
24 1.54666368845509
25 1.58798712459324
26 1.62872924143166
27 1.66971654616598
28 1.7094060391489
29 1.7483155087228
30 1.78964299863347
31 1.82821376384638
32 1.86667082762237
33 1.90424457608292
34 1.94203923183897
35 1.97970071236387
36 2.01742453794736
37 2.0557000760877
38 2.09328050987598
39 2.13096305248141
40 2.16997284142636
41 2.20688029365148
42 2.24306524374039
43 2.27859935790327
44 2.31828047966864
45 2.3539934358286
46 2.39093595260321
47 2.4268408199144
48 2.46096815252806
49 2.49673474346231
50 2.53160129716382
51 2.56527607898912
52 2.60181525595045
53 2.63464435043221
54 2.66969652390237
55 2.70360146478113
56 2.73600593266381
57 2.77901513880916
58 2.81192996093932
59 2.85228101115012
60 2.88790901361165
61 2.92135146417278
62 2.95679499593461
63 2.9908890348378
64 3.02211421052479
65 3.05411093059575
66 3.08586682840815
67 3.12033068403219
68 3.15124608884346
69 3.18426238969581
70 3.21744924210744
71 3.25018001574695
72 3.28062883220807
73 3.31997797224966
74 3.35917620621894
75 3.39739908827621
76 3.43283788279314
77 3.46416657711748
78 3.49885094101129
79 3.53518850027237
80 3.57110118872834
81 3.60358182315085
82 3.63514608507834
83 3.66776000856081
84 3.70920834636996
85 3.74268437191683
86 3.77615415478877
87 3.8064363841767
88 3.84477026480878
89 3.88180743758661
90 3.92217926251375
91 3.95357616984344
92 3.98482215581109
93 4.0201948389384
94 4.05319615322337
95 4.08408413510992
96 4.11344576700917
97 4.14567634093202
98 4.18079765971911
99 4.21651292252591
100 4.25177656151861
101 4.28506112241763
102 4.31858829018303
103 4.34872559753372
104 4.37880866007026
105 4.41147489512467
106 4.44865303625896
107 4.47907429391748
108 4.51153767958033
109 4.54714709644957
110 4.58625887407046
111 4.61989416464917
112 4.65279171893103
113 4.68922274213164
114 4.72368832953577
115 4.75471591290628
116 4.78377847281598
117 4.81708116209714
118 4.84746817855854
119 4.88248649317506
120 4.91056385817545
121 4.94216271583492
122 4.97449290269084
123 5.00906074289969
124 5.04009004783775
125 5.07223933454178
126 5.11020483348239
127 5.13893758649411
128 5.17107243984802
129 5.19900905005915
130 5.23499410450087
131 5.27784056273073
132 5.30496444518956
133 5.3395384263741
134 5.36662716621257
135 5.40354175535526
136 5.43811613747173
137 5.46814596821412
138 5.49545920714087
139 5.52821008569529
140 5.55358090763284
141 5.58288272533176
142 5.6116807189952
143 5.64090681764397
144 5.66926389481917
145 5.70103070875162
146 5.73278158586508
147 5.76178025794155
148 5.79774025514089
149 5.82951405270981
150 5.86121919656245
151 5.89045845679948
152 5.91510894256958
153 5.95686506500831
154 6.0005262314216
155 6.02592053749775
156 6.05602070845798
157 6.08862875528603
158 6.11915091546297
159 6.1455346076213
160 6.17412105221891
161 6.20077364904377
162 6.23099448478115
163 6.25445387913773
164 6.28493987469188
165 6.31204840353824
166 6.34781469219965
167 6.38513969957218
168 6.40759112489593
169 6.43358736438007
170 6.46767315034926
171 6.49863137416105
172 6.52364067026283
173 6.56210846223627
174 6.59348423420845
175 6.62013501780566
176 6.64635243352428
177 6.67246282594258
178 6.7226677769916
179 6.75394268650493
180 6.79524434764393
181 6.82166497562361
182 6.84832149356551
183 6.87940545660167
184 6.90297270493161
185 6.94199850063494
186 6.96885058725051
187 6.99640296231575
188 7.02532534411742
189 7.04724625119864
190 7.07295557990541
191 7.10161185498223
192 7.12835038354865
193 7.15708117568753
194 7.18934932014643
195 7.2122056080564
196 7.24531079400192
197 7.2727187404327
198 7.29953350992582
199 7.33251405815771
200 7.35663508219945
201 7.37773953739179
202 7.40504880792957
203 7.42465535810179
204 7.45131638350438
205 7.49679021637363
206 7.52485697712183
207 7.55940501568797
208 7.58869488073948
209 7.62471706307497
210 7.66208663828742
211 7.68650775532741
212 7.71065517515425
213 7.74617890546353
214 7.77627769745855
215 7.80205142902031
216 7.83707838278608
217 7.87927306963241
218 7.89877331152267
219 7.92049321414048
220 7.93947196782522
221 7.96398294995315
222 8.01265441411319
223 8.04894127281311
224 8.0900702537206
225 8.12344929018156
226 8.15092312266642
227 8.18431335800632
228 8.20594817356201
229 8.25930074526923
230 8.28686826621012
231 8.30714304296469
232 8.33953949103878
233 8.36127104272442
234 8.38616702995907
235 8.41310235385511
236 8.43981708258948
237 8.46284813067514
238 8.4887059885517
239 8.52260795522013
240 8.56321555987741
241 8.6026856625891
242 8.63803381438612
243 8.66760862283021
244 8.68777878167287
245 8.70922222220491
246 8.72855659580055
247 8.7571810865634
248 8.79178321627629
249 8.82633422697341
250 8.85144056783093
251 8.88252310953084
252 8.91083872824523
253 8.93600249759759
254 8.97292953257998
255 8.99779836945183
256 9.02428893233283
257 9.04984286667648
258 9.07893665532213
259 9.11784169538854
260 9.13618593930167
261 9.16966812190421
262 9.19798424394547
263 9.21816079959653
264 9.23539966091171
265 9.25825032113175
266 9.27747271498963
267 9.29968932753353
268 9.3232831853586
269 9.33786964797509
270 9.36789490704843
271 9.40408562256662
272 9.44277066091869
273 9.47089101180484
274 9.49052906102604
275 9.52389534267246
276 9.55834876238388
277 9.57999161101145
278 9.5961981539677
279 9.619833660084
280 9.64712543227655
281 9.6816217452626
282 9.72527726531415
283 9.7555078369636
284 9.77630871579773
285 9.80606983425283
286 9.82468889281837
287 9.869346871165
288 9.9113216490931
289 9.9351376686345
290 9.96333292535595
291 9.98973466136563
292 9.99555629967086
293 10.0239626877498
294 10.0455347875707
295 10.0649339723992
296 10.0817621037582
297 10.1030066761702
298 10.1297905025853
299 10.1531355034153
300 10.1787461191576
301 10.1996875338454
302 10.2268531100099
303 10.2616622102353
304 10.3267696727436
305 10.3612189122273
306 10.3784871264705
307 10.4100315332939
308 10.4468835360734
309 10.4635714062472
310 10.4989854150395
311 10.5426021727137
312 10.5882547103768
313 10.6035449798739
314 10.6173870994098
315 10.6320803205392
316 10.6395986057458
317 10.6531771025042
318 10.6728579507978
319 10.6933044287684
320 10.7106331715748
321 10.7387669803805
322 10.7673961271984
323 10.8077470213044
324 10.8315045355708
325 10.8646815026323
326 10.8750251693314
327 10.8990499110029
328 10.9270959664196
329 10.9602687555005
330 10.9986315046526
331 11.0267519534018
332 11.0454556716818
333 11.0801374553714
334 11.0874911339946
335 11.1194517819585
336 11.1633055713552
337 11.1950188562881
338 11.2226725918514
339 11.2599894421303
340 11.2814850244231
341 11.2993067204767
342 11.3173271713032
343 11.3350005521521
344 11.3481482112235
345 11.3715720822243
346 11.404254288842
347 11.4418330335412
348 11.5039737674785
349 11.549233531835
350 11.6002487274015
351 11.661804161577
352 11.6791279512304
353 11.7052267947121
354 11.7484190612943
355 11.7739091848924
356 11.8175780263717
357 11.8449688669932
358 11.8881089889546
359 11.9194355436287
360 11.9458539133866
361 11.9632346651613
362 11.9930858650219
363 12.0095322629147
364 12.0526098276789
365 12.0931556482481
366 12.1134757086588
367 12.1209836034124
368 12.147495572407
369 12.1995856553724
370 12.239729278151
371 12.2732632613564
372 12.2949909874265
373 12.3182991637482
374 12.3476628942893
375 12.3692429329637
376 12.4059768352243
377 12.4353834477843
378 12.4669300907321
379 12.492051857358
380 12.5204629933373
381 12.5755159274927
382 12.6164714619526
383 12.6347870093476
384 12.680092159372
385 12.6932650264676
386 12.7108444152383
387 12.7315743673786
388 12.7586524843028
389 12.7933994846282
390 12.835919270959
391 12.86119628573
392 12.9156895437538
393 12.9397232957154
394 12.9614420703063
395 12.9850644047695
396 13.0039662187849
397 13.0193831000441
398 13.0333235690946
399 13.0762153600558
400 13.1106246526569
401 13.1364826918286
402 13.1717455354759
403 13.208730768103
404 13.2346604450173
405 13.2849658070565
406 13.2925142607659
407 13.3295658339927
408 13.3616640910861
409 13.3743399145558
410 13.3880511990447
411 13.3961899217953
412 13.4308569822352
413 13.4616587962772
414 13.4796477146258
415 13.4976837560479
416 13.5274877992679
417 13.5367845971465
418 13.5692986655701
419 13.5991957642321
420 13.6502996812056
421 13.6693306992804
422 13.721708168759
423 13.7759757907339
424 13.8101195517417
425 13.8314145176301
426 13.8500175914896
427 13.8699495777805
428 13.8842678205388
429 13.9224442654778
430 13.9370139940201
431 13.9637250017068
432 13.9775251053166
433 13.9775133623988
434 13.9836422473939
435 13.9842455248902
436 14.0095123371212
437 14.0469723748958
438 14.0645913392015
439 14.0937479044976
440 14.1311865492526
441 14.1973396593252
442 14.2309051312982
443 14.2628079590481
444 14.2955197402977
445 14.3110407261549
446 14.3560055982706
447 14.3690200556054
448 14.3830692862957
449 14.4136880842243
450 14.445709840778
451 14.4588481488209
452 14.4782362977295
453 14.5138949665094
454 14.5438148533056
455 14.5602876920901
456 14.6033094634365
457 14.6274428261305
458 14.6446755518297
459 14.6690082533446
460 14.7183755822712
461 14.7623453828311
462 14.800127579658
463 14.8230237688708
464 14.8634463722524
465 14.8887234794607
466 14.9300174227702
467 14.9646223567458
468 14.9754830759565
469 15.0104411495923
470 15.0299762324059
471 15.0557013519811
472 15.0828162757523
473 15.1139845666696
474 15.1316171171165
475 15.1537748447949
476 15.158428404143
477 15.1770625315916
478 15.200342530552
479 15.220589425975
480 15.2513383937677
481 15.2817242384035
482 15.3049941392537
483 15.3166107181919
484 15.3249954840021
485 15.3797303241208
486 15.4116631699606
487 15.4551185377801
488 15.4695991191744
489 15.4824990849922
490 15.4934143216336
491 15.5094805774486
492 15.5128351261535
493 15.5253435279787
494 15.5956959992291
495 15.6120293994213
496 15.6380228545979
497 15.6863629780126
498 15.7136971323411
499 15.7256489454792
500 15.7654143176637
501 15.824233826357
502 15.8537474255391
503 15.8892903997691
504 15.9294820247198
505 15.9641238498502
506 16.0116254789251
507 16.01899897674
508 16.0454058568437
509 16.0626555978944
510 16.096204243352
511 16.1248809205775
512 16.2018121280465
513 16.2428267065679
514 16.277395421572
515 16.2925049049401
516 16.3242626393774
517 16.3620819401977
518 16.3904600126223
519 16.4405631367698
520 16.4679745747308
521 16.4920501276596
522 16.5223793821855
523 16.5401141592332
524 16.5630264393443
525 16.5886144643669
526 16.6359326020338
527 16.6538223795806
528 16.6651290822463
529 16.6977544921773
530 16.7091868724796
531 16.7412646767718
532 16.7742686669227
533 16.7969005597719
534 16.8169525501911
535 16.8504611469786
536 16.8606181819089
537 16.8955360818857
538 16.9255215633086
539 16.970634798072
540 17.0143895741814
541 17.048353367973
542 17.0762709049611
543 17.1339240653083
544 17.1559281220508
545 17.1715936581015
546 17.1932275726784
547 17.2093919871345
548 17.2235826298366
549 17.2338313028165
550 17.265961390938
551 17.2924478960568
552 17.3259092444981
553 17.3800015209027
554 17.4160145339034
555 17.4336944592215
556 17.4526704346327
557 17.4986415741512
558 17.5129567017901
559 17.5344129265956
560 17.5647734542376
561 17.5724394606048
562 17.6147846957514
563 17.6218359444464
564 17.6296026970248
565 17.6442659052929
566 17.6701068168378
567 17.7130805099068
568 17.7088830094858
569 17.7210575602282
570 17.7385772466102
571 17.7663720999776
572 17.7799634692072
573 17.8167264507194
574 17.8356793456053
575 17.860761102348
576 17.8689190326407
577 17.8900573774369
578 17.9116154862984
579 17.9530146642894
580 17.99610629469
581 18.008485537302
582 18.0563189354556
583 18.0632039613001
584 18.0905077168766
585 18.1123237819243
586 18.1271938602654
587 18.1816638201868
588 18.2118067753023
589 18.2852234378909
590 18.3555940737656
591 18.3682517743246
592 18.3961528688159
593 18.4080223763928
594 18.430469171461
595 18.4555469287022
596 18.4860962608125
597 18.4930601182656
598 18.5267665191845
599 18.5450332461884
600 18.5489442363753
601 18.5769718557066
602 18.6037351148259
603 18.6460901160321
604 18.66670424749
605 18.6753436073862
606 18.6946715720314
607 18.7031486041301
608 18.7283724728484
609 18.7332251115753
610 18.7568179013347
611 18.8068783016137
612 18.8342356635047
613 18.8471541306297
614 18.8511088660649
615 18.8734221350203
616 18.8853476536636
617 18.926947887489
618 18.9664102929663
619 19.0301367842649
620 19.0828063538835
621 19.11100830093
622 19.1220100636736
623 19.1403980080614
624 19.1798953775361
625 19.2287433719414
626 19.2884935658092
627 19.3190093629363
628 19.3475409855883
629 19.3778714668242
630 19.4011379450301
631 19.410489888643
632 19.4362151291103
633 19.4551037871265
634 19.4841365171326
635 19.5104129505057
636 19.5091366635197
637 19.5394875840806
638 19.5582013798144
639 19.5889761496385
640 19.5818908157513
641 19.6003580692885
642 19.6370256549007
643 19.6481382643432
644 19.6769848487689
645 19.7355003157037
646 19.7551490907814
647 19.7783909169162
648 19.7956521687954
649 19.8120208272397
650 19.8287431281065
651 19.8927763071089
652 19.9310306559503
653 19.9599587011574
654 19.9726197460563
655 19.9668912421363
656 20.0155352059718
657 20.0329962399887
658 20.0682693632572
659 20.1428847515702
660 20.1560509588214
661 20.1652989191533
662 20.1763798170973
663 20.1717718808735
664 20.2004512584316
665 20.2386710071203
666 20.2501841989579
667 20.2714503637326
668 20.3256930558207
669 20.3511889955217
670 20.4218955132712
671 20.4316298570686
672 20.4247304449874
673 20.4797209432592
674 20.5055182347129
675 20.5489889606223
676 20.5704525905262
677 20.6049043541872
678 20.6184671937823
679 20.6268907981604
680 20.652636785901
681 20.6548488645083
682 20.687175871909
683 20.737597601798
684 20.7622450714569
685 20.7842340500928
686 20.8748519023108
687 20.8998210479462
688 20.9258514058051
689 20.9660947290088
690 20.9828432257008
691 20.9910520952508
692 21.0285637242967
693 21.0693789396753
694 21.0888214441028
695 21.1413556178987
696 21.1817451707759
697 21.2068399362741
698 21.2471200896409
699 21.2803989619839
700 21.3172015368446
701 21.3254966091701
702 21.3199272158574
703 21.3131668633143
704 21.2990334889193
705 21.3078834931181
706 21.3642204574976
707 21.4053094394562
708 21.4431644965622
709 21.4765961371715
710 21.471854965994
711 21.4870702837499
712 21.5028106326884
713 21.535234726288
714 21.5500214391404
715 21.5517567196326
716 21.5895263043403
717 21.5947038126958
718 21.641199593081
719 21.6665951918922
720 21.6804184803185
721 21.6826750696889
722 21.7183344870354
723 21.7332419499562
724 21.7538919288677
725 21.7974169882048
726 21.8447807273493
727 21.865670563106
728 21.9006298314643
729 21.9247465053812
730 21.956325876656
731 21.9891783276336
732 22.0025954397594
733 22.0476177119521
734 22.0809312062502
735 22.126288991718
736 22.1469314838645
737 22.16054885794
738 22.1548631606564
739 22.1758513199591
740 22.1966077283896
741 22.2549647054481
742 22.2790223406454
743 22.2910751204402
744 22.3004324509701
745 22.3064254597542
746 22.2976529681553
747 22.3128724650353
748 22.3175745696348
749 22.3488411428874
750 22.3786725891093
751 22.4116300146231
752 22.416722230565
753 22.4699807041433
754 22.5231075936019
755 22.5586000560632
756 22.5659391372824
757 22.5877625565029
758 22.6107111228266
759 22.6223417397484
760 22.6498863537711
761 22.671484524736
762 22.7100097234376
763 22.7338266123539
764 22.7496691913689
765 22.7370193770834
766 22.7432127010833
767 22.7567421765166
768 22.7688436779223
769 22.7666797264321
770 22.774625908194
771 22.7848757336697
772 22.8351574629034
773 22.8652853327374
774 22.8691521016447
775 22.8986026080396
776 22.9124083478939
777 22.9180741831945
778 22.9663444380759
779 23.002212002123
780 23.0346041023221
781 23.0970435652007
782 23.1619317053991
783 23.1640956469699
784 23.1870342973411
785 23.2046801069862
786 23.2143699037887
787 23.2611822251154
788 23.2536020397771
789 23.2839354369447
790 23.3376022466779
791 23.3309688755891
792 23.3861963074787
793 23.4081236588493
794 23.4415370902797
795 23.5021139779643
796 23.5237806040187
797 23.5534739054339
798 23.5785711399792
799 23.5981827521978
800 23.6193432277119
801 23.6049057074965
802 23.6031522916096
803 23.638617644572
804 23.660514809013
805 23.6715638260773
806 23.6910079169575
807 23.7184813907323
808 23.7482913464028
809 23.7666726748534
810 23.7923261846141
811 23.8388981737258
812 23.8504656590764
813 23.8584053826651
814 23.8732079050166
815 23.9474684244968
816 23.9878111124474
817 24.0222218626761
818 24.0704713203528
819 24.1321784018078
820 24.18417288511
821 24.2091079882613
822 24.2338366255062
823 24.2737141713278
824 24.2948070299143
825 24.2992440429749
826 24.3233049548512
827 24.3385872051493
828 24.3652552237089
829 24.3782255498393
830 24.3914472022706
831 24.4103101597989
832 24.4054011406897
833 24.4113183355759
834 24.4476938317528
835 24.4637828320657
836 24.5451370003023
837 24.5664046107113
838 24.621128611169
839 24.6158747675731
840 24.6393915886507
841 24.6467253831322
842 24.6604471659497
843 24.6903129081231
844 24.7410550211873
845 24.8335156283709
846 24.8643506352894
847 24.8659019316108
848 24.8744492692038
849 24.884024224228
850 24.9347623978399
851 24.9610101512543
852 25.02273755319
853 25.0469853699168
854 25.0574504275715
855 25.0760502878715
856 25.0801205340721
857 25.0667890116344
858 25.109507988095
859 25.1106472564243
860 25.1084466964692
861 25.1082294086516
862 25.1216264414142
863 25.2152385182575
864 25.2807803175307
865 25.3341583843698
866 25.3424058991767
867 25.3400948969955
868 25.3741723810896
869 25.3832219354911
870 25.4077661740936
871 25.4564685303224
872 25.4972028530519
873 25.5208088181613
874 25.5578648847518
875 25.5929869914697
876 25.6305064557911
877 25.6438486148928
878 25.6533932744229
879 25.6631470811682
880 25.6500687224424
881 25.6941747712858
882 25.7400894319215
883 25.7539127177864
884 25.8499239704913
885 25.9182196529029
886 25.9654995149397
887 25.9675229988604
888 25.980860461996
889 26.0122007056963
890 26.074509710552
891 26.0835314561368
892 26.07168529499
893 26.0809282302449
894 26.1180058090881
895 26.1482633048013
896 26.1747119694569
897 26.1940638424316
898 26.1950625765962
899 26.2028475486024
900 26.2687563215032
901 26.2830450243414
902 26.3268379423061
903 26.3359807144274
904 26.3332102570557
905 26.3472686047069
906 26.4117294480648
907 26.4480119690137
908 26.4810258550569
909 26.5184619038173
910 26.5719647277466
911 26.5756448819771
912 26.6207490599276
913 26.6154105844036
914 26.6348963251601
915 26.633050320081
916 26.6142078424961
917 26.6691547329838
918 26.6817083279987
919 26.6798363774572
920 26.6919100555555
921 26.7066225310413
922 26.7268441499951
923 26.7573813571719
924 26.7937047045172
925 26.808216418489
926 26.8351116229953
927 26.8120719705788
928 26.8021036798143
929 26.8368631219644
930 26.8454556521653
931 26.8464110295376
932 26.913833400242
933 26.9607938855057
934 27.0627920182155
935 27.0816870099868
936 27.1367667114191
937 27.164642924163
938 27.1888290249485
939 27.2390717053881
940 27.2576317607937
941 27.2767084296848
942 27.3042543087232
943 27.3117627733561
944 27.3152693631595
945 27.3961388325479
946 27.4114645762012
947 27.4363477234331
948 27.4442433355722
949 27.4511125433032
950 27.4794671184829
951 27.4963720464495
952 27.5210748009088
953 27.528666995751
954 27.5407247842808
955 27.5734127607156
956 27.5642112259835
957 27.5638779794197
958 27.5606705945663
959 27.5388799698491
960 27.5089732115139
961 27.5160833103482
962 27.5154128000447
963 27.5449739561753
964 27.5730467690672
965 27.6126641634863
966 27.6256270941024
967 27.6330852346094
968 27.6568257343177
969 27.6747244149795
970 27.7093181010609
971 27.7626024416074
972 27.7862961360992
973 27.794775381976
974 27.8009969466103
975 27.805398865757
976 27.8295123502701
977 27.8417815522515
978 27.8764042162288
979 27.9009521473663
980 27.90700140927
981 27.9455982246465
982 27.9450708448734
983 27.987476309394
984 28.0185983155053
985 28.0664608881246
986 28.0992559992034
987 28.1062612991088
988 28.1242982033144
989 28.113499525802
990 28.1059433010296
991 28.1559713468315
992 28.1802432650728
993 28.2357533868725
994 28.245756822382
995 28.2811141131863
996 28.358881759371
997 28.4047187805167
998 28.4642527750155
999 28.4646633567628
1000 28.4820653589607
};
\addlegendentry{kernel kerding}
\addplot [semithick, color1]
table {%
1 0.255031946981115
2 0.353906220052934
3 0.440275440907041
4 0.516428725054902
5 0.586455292178351
6 0.648820982592984
7 0.707088958555637
8 0.762429505198485
9 0.815548212152431
10 0.866138637669517
11 0.916321785615136
12 0.961845795788531
13 1.0073052681182
14 1.05242928118828
15 1.0998919388423
16 1.14395102495867
17 1.18614594692518
18 1.23528786989815
19 1.27565945386577
20 1.31508977470906
21 1.35219694752218
22 1.39094939223965
23 1.42651458693042
24 1.46539052696395
25 1.50636019511783
26 1.54206475576714
27 1.57999531208685
28 1.61767211002782
29 1.65319934437288
30 1.69135135588917
31 1.73001579542788
32 1.76543947538938
33 1.80395404234814
34 1.84690620995318
35 1.8844566848001
36 1.91716025911642
37 1.95487512501272
38 1.99259952375837
39 2.0272074168037
40 2.06639685925062
41 2.09993362132563
42 2.14572682158855
43 2.18402994350635
44 2.2194629792867
45 2.25305086719294
46 2.29376874732927
47 2.33168001138183
48 2.36460817212512
49 2.39966399075149
50 2.42619861826857
51 2.46029778711717
52 2.49023792122006
53 2.51716841339134
54 2.54710187123344
55 2.5800221713
56 2.61202328300545
57 2.64611951861419
58 2.68518512484874
59 2.72096458085276
60 2.74540339005937
61 2.77697947617216
62 2.81357593556094
63 2.85822602093166
64 2.89093434266816
65 2.92199991022827
66 2.95319554173925
67 2.98057253979469
68 3.00956069793479
69 3.0461405054673
70 3.08808973196244
71 3.12328767214734
72 3.16010999982705
73 3.19032546698778
74 3.22421810131623
75 3.25871066474873
76 3.29260668470417
77 3.3265435460269
78 3.35185682064937
79 3.38726169256905
80 3.41867693100947
81 3.43945571500794
82 3.47953459350069
83 3.50436888614581
84 3.54136291619594
85 3.57275459622721
86 3.60110363532948
87 3.63315590983077
88 3.67475474799212
89 3.70360063288436
90 3.73294044340136
91 3.77016489368358
92 3.79495753088605
93 3.81533356873761
94 3.83363717232898
95 3.85284196350979
96 3.8884344887988
97 3.91183214494438
98 3.94543654280635
99 3.97653141529884
100 4.00438732784579
101 4.04098530511997
102 4.08559291707986
103 4.1054587730195
104 4.12862298681737
105 4.1543555589859
106 4.18612790425058
107 4.22005878830061
108 4.25028036224494
109 4.28391459995422
110 4.33542835746599
111 4.36992307195318
112 4.39197085500497
113 4.41539045486475
114 4.4506522690625
115 4.47229568686151
116 4.51691894484219
117 4.53514497388601
118 4.54566586665665
119 4.57746983951761
120 4.62320316548623
121 4.65593076239786
122 4.67828660893418
123 4.71975818367565
124 4.74604061919896
125 4.76722772051798
126 4.79060046233165
127 4.810698457428
128 4.83888644158977
129 4.8665442981631
130 4.90268511208188
131 4.93637899104942
132 4.96147218509964
133 4.9898686143909
134 5.01392315966372
135 5.03999362396251
136 5.06723217376049
137 5.0961669666538
138 5.12065268874137
139 5.14722086005779
140 5.18525701929621
141 5.21675673702994
142 5.24490018525932
143 5.27815637474653
144 5.30293383325868
145 5.33643566990612
146 5.37644501907564
147 5.41355068849051
148 5.44097469962587
149 5.45688995016276
150 5.47632636079014
151 5.50644190115386
152 5.52694058849664
153 5.55993978581588
154 5.60279859505171
155 5.63409964760681
156 5.64995716950672
157 5.67651736342097
158 5.71127740696882
159 5.72270015114463
160 5.75881733153564
161 5.79688710728785
162 5.81692098515028
163 5.85865946758902
164 5.87498646520756
165 5.90155785342366
166 5.93216200789618
167 5.95654387081305
168 5.97707834526551
169 5.99750856783975
170 6.02132336021332
171 6.04068625605272
172 6.07585700157114
173 6.09274639869257
174 6.10309659341082
175 6.11286448626161
176 6.12462528218735
177 6.14628654829615
178 6.17073913177987
179 6.18765678646376
180 6.18706514005738
181 6.20121408459818
182 6.21915579104252
183 6.24782384142421
184 6.25377716064768
185 6.25381180625709
186 6.28814983948037
187 6.31365902725324
188 6.34706853716769
189 6.3658658948715
190 6.39591012554401
191 6.41396190983961
192 6.43254318816258
193 6.46370186671493
194 6.49472402283004
195 6.51029145395967
196 6.52635642713398
197 6.5329577622237
198 6.57423878446886
199 6.59874019575536
200 6.61682793411294
201 6.63769058542534
202 6.68286489334771
203 6.72241078939475
204 6.74253327120864
205 6.76583964277589
206 6.78636619787328
207 6.80015010697838
208 6.81510370711299
209 6.83018650313079
210 6.85975602992537
211 6.88532829995615
212 6.90745330975072
213 6.91823582619042
214 6.91355604378465
215 6.94101130970068
216 6.96991402523872
217 6.9933688077828
218 7.01105498698483
219 7.05957139373687
220 7.10259951296588
221 7.13357128529397
222 7.17162495135684
223 7.18615195284978
224 7.19939361751899
225 7.21442377455187
226 7.22358729710255
227 7.25232007548223
228 7.25582001292699
229 7.26020352786027
230 7.25651346707537
231 7.27990866789006
232 7.28000058809407
233 7.30431487912737
234 7.29791857610361
235 7.32535038562405
236 7.34745103082275
237 7.36146317793865
238 7.39065526876814
239 7.42205250784486
240 7.44014249556947
241 7.43369099030439
242 7.46309555366588
243 7.48000930837497
244 7.50468829484345
245 7.53777344949757
246 7.55764844827511
247 7.57870960040835
248 7.62388842337371
249 7.64952830060167
250 7.66939818899365
251 7.69673990411685
252 7.72221519228839
253 7.72891813651361
254 7.76325181896099
255 7.77056867588679
256 7.78771484292633
257 7.80547112710016
258 7.82532258916903
259 7.86875572209723
260 7.89804441058306
261 7.92459930036552
262 7.98008672457301
263 8.01680861186844
264 8.04340588345923
265 8.07120445710947
266 8.11114617190652
267 8.15136916524659
268 8.21388908080792
269 8.25095253945158
270 8.27292279754458
271 8.29220239991293
272 8.31620343213135
273 8.31808566230427
274 8.33824952786604
275 8.31576230504504
276 8.35266115818415
277 8.36186317068313
278 8.38278475513144
279 8.39899638753299
280 8.40942634820047
281 8.43515344707657
282 8.44613114733558
283 8.45771905278582
284 8.44982564395257
285 8.46090925784223
286 8.49062922254195
287 8.52349250004691
288 8.52867662290795
289 8.53227965421834
290 8.55979985783335
291 8.59168943634318
292 8.62711273053972
293 8.66042373526311
294 8.69411731757354
295 8.71092799309044
296 8.72515798624519
297 8.73223874672608
298 8.76905158954337
299 8.78468449139873
300 8.81343024267115
301 8.83174533500664
302 8.82739935066819
303 8.83549505372503
304 8.87066373122029
305 8.86815212245652
306 8.89475285273489
307 8.91863147289456
308 8.92804718915569
309 8.91577275250316
310 8.94428274438905
311 8.95768464539153
312 8.95832285973235
313 8.98594501024062
314 9.00435083089235
315 9.00164316866841
316 9.03439890888645
317 9.04650797964046
318 9.04905839422244
319 9.07568433400502
320 9.03927760449517
321 9.02124892818932
322 9.0356809064235
323 9.05643631044436
324 9.115055845728
325 9.15933538569359
326 9.19728654167075
327 9.25319630920247
328 9.28790430922343
329 9.29302526664861
330 9.29775912497738
331 9.29215186019523
332 9.31058372606755
333 9.34329343859419
334 9.36464502133593
335 9.39982785449688
336 9.42918768468379
337 9.43973050298609
338 9.4546426620386
339 9.45946504647819
340 9.50036678646052
341 9.51031646417383
342 9.53108440661708
343 9.53212611128853
344 9.58032767748192
345 9.60122610790629
346 9.63988889847601
347 9.6734410496811
348 9.67587654807442
349 9.70398921378054
350 9.7278775354653
351 9.74560409165428
352 9.74696489152031
353 9.76319910145856
354 9.79458025888076
355 9.80740906154428
356 9.81062417291303
357 9.83622614818142
358 9.85012094370268
359 9.85900134505972
360 9.87109582542017
361 9.88731734638643
362 9.91367025010951
363 9.9572498398997
364 9.99587840629437
365 10.0175518106086
366 10.0259345283904
367 10.0619997783622
368 10.0757353483065
369 10.1121760601387
370 10.179025577465
371 10.193302972666
372 10.1917932691729
373 10.1763773231666
374 10.1874207750857
375 10.2016004673357
376 10.210210112441
377 10.2004227187641
378 10.2270114701191
379 10.2528897239933
380 10.273462140958
381 10.2804325808853
382 10.2918301928903
383 10.3214581060776
384 10.3336157853313
385 10.3520102385375
386 10.3503569299924
387 10.3631517220879
388 10.3453605602946
389 10.3544564040307
390 10.339674963176
391 10.3690393625958
392 10.3427266526269
393 10.3662011762059
394 10.3852673806962
395 10.4078726433625
396 10.4576678836858
397 10.5019658810547
398 10.5097196790548
399 10.5207833189228
400 10.5201993041182
401 10.5254207690642
402 10.5153751657916
403 10.5006780550367
404 10.516799575097
405 10.5401320730003
406 10.5650261083907
407 10.5843400251458
408 10.575096390062
409 10.5747000266811
410 10.6085777864331
411 10.6102810319073
412 10.665262507153
413 10.6909425307032
414 10.7617876644634
415 10.8295812759854
416 10.8463804436072
417 10.8314482128625
418 10.8286161597224
419 10.823145063742
420 10.7911908187533
421 10.7841420706151
422 10.7984695191976
423 10.8054517679726
424 10.8019014877085
425 10.8233334323148
426 10.7859206533786
427 10.8155498086032
428 10.8389604839366
429 10.8238819977703
430 10.8372653529214
431 10.8378624512428
432 10.8744877292312
433 10.8866891036525
434 10.9146815883777
435 10.9342692748293
436 10.9467968298273
437 10.9645291609274
438 10.973428199451
439 11.0035043862784
440 11.0360508924805
441 11.0248479745965
442 11.0204260914585
443 11.0397395496866
444 11.0520083127396
445 11.0868825243914
446 11.0939956350569
447 11.0954630922237
448 11.1228574457542
449 11.1216375231693
450 11.1270592525892
451 11.1427867761302
452 11.155788801726
453 11.1551963880444
454 11.1730963802345
455 11.1735186839941
456 11.174934504246
457 11.1984018473625
458 11.2186741048468
459 11.2025376419038
460 11.1943152138341
461 11.2103842255982
462 11.2402623254688
463 11.242583387014
464 11.2651903122859
465 11.2411148859729
466 11.2584412364238
467 11.2808282272302
468 11.2716656639861
469 11.3168245799572
470 11.3724323247948
471 11.3310732190721
472 11.3207195182746
473 11.3062620676579
474 11.3217698442744
475 11.3688685889579
476 11.4092665477613
477 11.4000213047064
478 11.4066181541414
479 11.3991168443365
480 11.4211699622178
481 11.4290732361621
482 11.4506640065848
483 11.4651142159336
484 11.4568222214828
485 11.454114920259
486 11.4856824517987
487 11.4929043620803
488 11.5189035620592
489 11.523521091807
490 11.5277287394033
491 11.5190785287974
492 11.5574345737895
493 11.5187581569153
494 11.4950086190241
495 11.4812336021701
496 11.4710206152125
497 11.4411513224334
498 11.4734588204376
499 11.4610739611514
500 11.4736799127681
501 11.4644910865906
502 11.4689526476167
503 11.4858469980757
504 11.43634086234
505 11.4203481067807
506 11.4051770964938
507 11.3691398785466
508 11.3224504989156
509 11.339792301541
510 11.3576608135954
511 11.3704265542091
512 11.3954498877212
513 11.423467922294
514 11.431945494183
515 11.465767957585
516 11.473390727571
517 11.4898706934899
518 11.497244386994
519 11.4677974424284
520 11.4711465783125
521 11.4859176840007
522 11.5088371830305
523 11.5022858864919
524 11.4971286389417
525 11.5358485247614
526 11.557393173519
527 11.5795945285318
528 11.6123894427756
529 11.6273418891154
530 11.6242659112624
531 11.6281281395894
532 11.6663737980531
533 11.6971919077554
534 11.7186176207459
535 11.7445235600935
536 11.7741687308867
537 11.803640404183
538 11.824306753111
539 11.8491166334615
540 11.8218347007745
541 11.8704355709541
542 11.8678766424504
543 11.8394898166404
544 11.8269596618543
545 11.855764635069
546 11.8225632002833
547 11.8067486376391
548 11.8036394522348
549 11.7755723740949
550 11.7720448372394
551 11.7627433533962
552 11.761198073232
553 11.7866824039704
554 11.8331109062578
555 11.8587477378493
556 11.885240580858
557 11.9045395134484
558 11.9193976623831
559 11.9345140692294
560 11.9666814625651
561 12.0121363904418
562 12.0107636251903
563 11.9989506236241
564 12.0306781314138
565 12.0062208646067
566 12.0459449518505
567 12.0259932206542
568 12.0127981209032
569 11.9819544265395
570 11.9858205839446
571 12.0081760218022
572 12.0220585719997
573 12.0408061280892
574 12.0478947642609
575 12.0646663507078
576 12.0649570537792
577 12.0879042233157
578 12.0904166415002
579 12.1032051743448
580 12.117696686064
581 12.1367875882271
582 12.1779948461108
583 12.182959455366
584 12.1737280927673
585 12.1898079452638
586 12.1798129975628
587 12.2021726519913
588 12.2162790303648
589 12.2476912155205
590 12.2499636929248
591 12.267012226017
592 12.2364940541311
593 12.2267626038132
594 12.2288247457117
595 12.2433586138812
596 12.2709146165036
597 12.2945571930619
598 12.2718473928089
599 12.3079171725579
600 12.2873998562465
601 12.2670218534634
602 12.2851524721823
603 12.2999927230636
604 12.2866147067035
605 12.277539991482
606 12.3126234109854
607 12.3454717777052
608 12.3538099309729
609 12.3812454311047
610 12.3880987547754
611 12.3762304936231
612 12.3744695812561
613 12.3582809519834
614 12.3713999100225
615 12.3773000540647
616 12.3644060840205
617 12.4065109627182
618 12.4090826262098
619 12.4243233065093
620 12.4503712491534
621 12.4780223108131
622 12.4834423917648
623 12.5046316972951
624 12.5174734150175
625 12.5244927663328
626 12.5313573483867
627 12.5256650107603
628 12.5559849199666
629 12.5628169587222
630 12.5760917609073
631 12.616252320679
632 12.656435549613
633 12.6340040504775
634 12.6420176594768
635 12.6589838337627
636 12.7121817983102
637 12.6951435172177
638 12.686095219327
639 12.6996924222307
640 12.7166360987378
641 12.7141138302481
642 12.740319773953
643 12.7696201371444
644 12.8025976987365
645 12.8196610605156
646 12.8655928970071
647 12.9303717795145
648 12.947023937787
649 12.953403747579
650 12.9552408178902
651 12.9497731375696
652 12.9392010449043
653 12.92659484421
654 12.9308480692741
655 12.8899110430451
656 12.8455933058463
657 12.8189372291134
658 12.796117891097
659 12.8070616867661
660 12.8124661258664
661 12.8117033185196
662 12.7802724060902
663 12.7833102719765
664 12.7957515006914
665 12.7908366817077
666 12.7659317459443
667 12.8015421431183
668 12.8286050394288
669 12.8381353873551
670 12.8121060825202
671 12.7964930651846
672 12.8140062318001
673 12.777881525131
674 12.7811749372793
675 12.7855412641708
676 12.7808556971028
677 12.8071125380152
678 12.7945143207905
679 12.7958832838768
680 12.7927019146266
681 12.8096335860617
682 12.8371399242242
683 12.8097064858152
684 12.8018983063842
685 12.8082836981286
686 12.8451608041841
687 12.8732311040032
688 12.8949623277474
689 12.936711454605
690 12.9598328895966
691 12.9673982526531
692 13.0195048624229
693 13.0463759236423
694 13.0844181313289
695 13.0616667254679
696 13.0977984625262
697 13.1218024164726
698 13.129691189337
699 13.175336523361
700 13.1573822540181
701 13.1270398450299
702 13.1440318992488
703 13.1403643517423
704 13.147892618231
705 13.1729744324491
706 13.2068793988462
707 13.2134032035273
708 13.1885542247648
709 13.1868569239461
710 13.1989619928469
711 13.2346192286101
712 13.2529628819885
713 13.2453561545133
714 13.2460794409693
715 13.2555357450127
716 13.266751430248
717 13.2936565469179
718 13.3080163791297
719 13.29273538759
720 13.3139748630334
721 13.3238994270254
722 13.3475436702162
723 13.3096030381924
724 13.3140393990787
725 13.3148332682832
726 13.3122646262162
727 13.3203121920801
728 13.3124521593754
729 13.3098788834819
730 13.2993397016369
731 13.3237638341427
732 13.345143288089
733 13.338409590151
734 13.3554398948132
735 13.3647067742785
736 13.3856837496169
737 13.4111895197565
738 13.3757689559264
739 13.3805013229903
740 13.380046044498
741 13.3671241790805
742 13.3596970214367
743 13.3911739003333
744 13.4226209956989
745 13.4190129624551
746 13.4044634174647
747 13.4414459081948
748 13.4337848670736
749 13.4719880092198
750 13.4490192735265
751 13.4775884376965
752 13.493715731803
753 13.5076767218539
754 13.518306046124
755 13.5571726650086
756 13.5431171615561
757 13.5604900483867
758 13.5693777348869
759 13.5996870700379
760 13.5950702774627
761 13.6182666991001
762 13.582549818207
763 13.5547875969159
764 13.5946267116983
765 13.5669866020738
766 13.5422680438946
767 13.5719732974621
768 13.5619221715906
769 13.5869339238158
770 13.5793053498826
771 13.5670021341336
772 13.5784791481187
773 13.6093794814458
774 13.6065116361291
775 13.6457011402332
776 13.6850569669422
777 13.6692565431928
778 13.6402870793903
779 13.6592690087709
780 13.653676589077
781 13.6354587059373
782 13.668886007212
783 13.684692355161
784 13.6833181045522
785 13.7000384774249
786 13.6999094507712
787 13.6996227045082
788 13.6949394307431
789 13.7018432990487
790 13.7202325613894
791 13.727644363618
792 13.7380570010682
793 13.7146944402615
794 13.7449395700539
795 13.7407858014237
796 13.7311831818148
797 13.7555036009796
798 13.7747093518886
799 13.7745034023858
800 13.7610722436384
801 13.7449327434062
802 13.7342564460971
803 13.778079345693
804 13.803899144448
805 13.8033945529862
806 13.7805349363708
807 13.7525242694315
808 13.7650508004027
809 13.72942845324
810 13.7251543899653
811 13.7612540143625
812 13.7919507839989
813 13.7666236180589
814 13.776186437756
815 13.7717255312636
816 13.7675636199564
817 13.752371579175
818 13.7684608025338
819 13.8106212182843
820 13.8322338747723
821 13.850714781888
822 13.8569736989425
823 13.8554425342974
824 13.867358789648
825 13.8681907686102
826 13.8731327897144
827 13.8910343871132
828 13.9067060254103
829 13.9507680268007
830 13.927573294338
831 13.9155604597144
832 13.8977766084769
833 13.8960006649886
834 13.8937339565312
835 13.8819640999446
836 13.8944259006114
837 13.8853612080912
838 13.8722851208722
839 13.8904367303944
840 13.8953295054788
841 13.896546849311
842 13.9176685951122
843 13.8853652933883
844 13.8804851528951
845 13.8879036424086
846 13.8874256668218
847 13.8959297126679
848 13.87162478373
849 13.8750087431809
850 13.8505165626148
851 13.8855061691327
852 13.912548473543
853 13.9316382218216
854 13.9369341694455
855 13.9163270012212
856 13.9086821411661
857 13.9210361609056
858 13.9115376242824
859 13.9232600847084
860 13.9390145777611
861 13.9412753482601
862 13.9603643005991
863 13.9402511059198
864 13.9348246175027
865 13.9781442816057
866 13.9831987411603
867 14.0172876667345
868 14.049627241566
869 14.0589151428217
870 14.0729452879526
871 14.085039539754
872 14.1001492533678
873 14.108782117907
874 14.1277364080101
875 14.1436730908106
876 14.1469147006748
877 14.1872594094654
878 14.1953190082636
879 14.2187258595312
880 14.2382252953534
881 14.2662594771477
882 14.2854591585237
883 14.279025325257
884 14.2505721581932
885 14.224465378142
886 14.235630077479
887 14.2606714508252
888 14.2404817962489
889 14.247647471003
890 14.2156736513696
891 14.1985300714363
892 14.2249940497887
893 14.2297710102746
894 14.2279352196699
895 14.2679559298687
896 14.2798257198367
897 14.2936424614085
898 14.284931679496
899 14.2830163868566
900 14.2479057607489
901 14.2516418481274
902 14.2375441384029
903 14.2439349173728
904 14.2119256823979
905 14.2317551906258
906 14.2066477580103
907 14.1916438029907
908 14.1773110668879
909 14.1700831442328
910 14.1805751122966
911 14.1547485550114
912 14.1239564652281
913 14.1095749993599
914 14.1088455586548
915 14.1185472821798
916 14.1456661489149
917 14.1386791204062
918 14.1093180046723
919 14.1348035075761
920 14.1391722803517
921 14.1412301594575
922 14.1318139484559
923 14.1208211562074
924 14.1174218866852
925 14.0798308502587
926 14.0893290321693
927 14.0964835537627
928 14.0817420973987
929 14.0678603583741
930 14.0616373424181
931 14.035484595069
932 14.0308933708928
933 14.060113773514
934 14.0712745907035
935 14.0817581652966
936 14.1084171518899
937 14.1104318877921
938 14.120390421154
939 14.1044134942543
940 14.0736345737024
941 14.053423357213
942 14.0600306983222
943 14.0659278693939
944 14.0329211456491
945 14.0191163444442
946 13.9923297361248
947 13.9811365573933
948 13.968626680319
949 13.9946199403919
950 14.0137441297072
951 14.0273655361639
952 14.0338299909977
953 14.0478645735608
954 14.0592293962329
955 14.0590625963915
956 14.0820149306854
957 14.1120500860323
958 14.1061018747492
959 14.1233244516291
960 14.1410708832205
961 14.1390466625612
962 14.1477970145846
963 14.1602877765666
964 14.1345680771896
965 14.1587639986414
966 14.1381443640507
967 14.1480281421471
968 14.1534524275355
969 14.1656440645407
970 14.1484787757595
971 14.1383295712092
972 14.1496126793958
973 14.1618736676685
974 14.1664857893174
975 14.1429604543625
976 14.1579899826644
977 14.1637424772536
978 14.1587721276064
979 14.1395884251579
980 14.1425983271482
981 14.1432209500017
982 14.1778393750506
983 14.1887764279541
984 14.2038754647886
985 14.1866088671172
986 14.1716650044319
987 14.1543594419038
988 14.1621800652029
989 14.1492302098931
990 14.1327089851442
991 14.1515381712971
992 14.1362243799294
993 14.1131933206626
994 14.0899969770056
995 14.1049662589836
996 14.1113682134599
997 14.0858397245906
998 14.1150368048155
999 14.1246992749997
1000 14.1284480278986
};
\addlegendentry{continuous herded Gibbs sampling}
\end{axis}



==> l2_error.tex <==
% This file was created by tikzplotlib v0.9.8.
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
label style={font=\footnotesize},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
legend style={font=\footnotesize},
log basis x={10},
tick align=outside,
tick label style={font=\footnotesize},
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={number of samples \(\displaystyle T\)},
xmin=0.707945784384138, xmax=1412.53754462275,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle L_2\) error},
ymin=0.185900117290448, ymax=1.39392216701664,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1,1.2,1.4},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,1.2,1.4}
]
\addplot [semithick, color0]
table {%
1 1.17737454220855
2 1.08960063117627
3 1.01861425278781
4 0.963365125920787
5 0.920506647556543
6 0.889631520142966
7 0.865190355363755
8 0.84707500975787
9 0.829853972185398
10 0.817048531966423
11 0.80310657304529
12 0.789227060485608
13 0.776945753526004
14 0.767378937985297
15 0.758361325343994
16 0.750863132452307
17 0.743166697072021
18 0.728274550087989
19 0.719800206861542
20 0.711195554674181
21 0.70359634110166
22 0.696174130683279
23 0.691413123478777
24 0.684001221557088
25 0.673959660112693
26 0.667838104765577
27 0.663302424188544
28 0.658712322272496
29 0.653435960487931
30 0.647960918570764
31 0.640836435470103
32 0.63438225027878
33 0.628954355212993
34 0.625809755686295
35 0.622377558478493
36 0.618533370779139
37 0.611089012701324
38 0.603877428771649
39 0.601328639281793
40 0.59630250730934
41 0.593570772788355
42 0.591771939603315
43 0.589760616342279
44 0.586812556900254
45 0.582307762821909
46 0.57921094642548
47 0.573155619755787
48 0.571233506682506
49 0.567982914003496
50 0.566483141311586
51 0.564351840189165
52 0.560671680530455
53 0.558305857093772
54 0.554117092491992
55 0.553881305235408
56 0.552474355410535
57 0.547715727162439
58 0.5450307112571
59 0.541440378742322
60 0.538343967181077
61 0.53577136275019
62 0.533687600562851
63 0.53140995414064
64 0.528738531252055
65 0.528789096545261
66 0.525847842900821
67 0.523186070432859
68 0.522442749982955
69 0.518952622702739
70 0.517517527452902
71 0.517015681814934
72 0.514750565283957
73 0.510847665025777
74 0.505527334888917
75 0.502296219132418
76 0.499431940999669
77 0.500065907067718
78 0.496661537841128
79 0.492768523990838
80 0.489661665328347
81 0.486535313916356
82 0.482861237450365
83 0.483224363463758
84 0.480476319354758
85 0.47799397543186
86 0.477258945678329
87 0.475767061188439
88 0.473871369700078
89 0.471589905272555
90 0.46683419940399
91 0.467234202593543
92 0.467170779187904
93 0.465930707846209
94 0.465408407955448
95 0.465017505868461
96 0.464137968287797
97 0.463136131763853
98 0.461928654837834
99 0.457162254870282
100 0.454891544169878
101 0.451780884548602
102 0.451132295659938
103 0.449338795066
104 0.448657206391093
105 0.448334729214635
106 0.446657544643712
107 0.44671113133189
108 0.444421304986594
109 0.443035006536349
110 0.438620508597846
111 0.43725058530601
112 0.436985056167856
113 0.436640773939356
114 0.435656988400035
115 0.432108301009783
116 0.431523637462757
117 0.429211097981936
118 0.428423810817017
119 0.428050400068244
120 0.427500848882082
121 0.427224978285896
122 0.427251525883148
123 0.42715654884416
124 0.42577538068268
125 0.425708986878241
126 0.42412031193429
127 0.422522340786632
128 0.422112623600934
129 0.421582615004463
130 0.419121872225947
131 0.417403372048105
132 0.418100490877741
133 0.415156474120662
134 0.416052724375893
135 0.414985017917518
136 0.413636449966492
137 0.413331834353908
138 0.414384608020551
139 0.414499398107122
140 0.413319306880154
141 0.412791583856489
142 0.412912345178775
143 0.412859456024545
144 0.412515216833729
145 0.41176670390187
146 0.410923890837751
147 0.409801220612387
148 0.408602113633355
149 0.407412479943204
150 0.406974077239912
151 0.405592607444056
152 0.406084738320605
153 0.4040420277319
154 0.402594957611378
155 0.40313734293815
156 0.402248798914348
157 0.40086225096528
158 0.400963790824264
159 0.399365473050368
160 0.398418704615184
161 0.397437875406537
162 0.397943834441816
163 0.397920984127998
164 0.397007613212557
165 0.395021655660672
166 0.394067449751879
167 0.393197383149568
168 0.393021019548369
169 0.392632521369615
170 0.390677998603095
171 0.391052357823965
172 0.389480785494525
173 0.388217035970802
174 0.388326375481123
175 0.388071501641096
176 0.3867377152314
177 0.387498380266002
178 0.385913105952927
179 0.385737636105761
180 0.385359916003368
181 0.385932835294405
182 0.386079971101161
183 0.384736801756822
184 0.38441317318134
185 0.384274088981145
186 0.384207198109563
187 0.385288170942274
188 0.385058055901441
189 0.384702262179905
190 0.385034418031853
191 0.384876149224432
192 0.384615158867496
193 0.384624685171115
194 0.383637694493772
195 0.383227869762886
196 0.383555519628121
197 0.382526582072476
198 0.382864297883061
199 0.38265056073142
200 0.381499749412307
201 0.381724254337286
202 0.382008305649854
203 0.381499517324134
204 0.381221726885856
205 0.378448087047232
206 0.377763202030019
207 0.377116540764475
208 0.37642463743263
209 0.375578130519682
210 0.375149653693017
211 0.375039141999069
212 0.375425335265516
213 0.373092993974939
214 0.373047488958697
215 0.372446598660592
216 0.372184566583631
217 0.371528786044881
218 0.371997682099409
219 0.371803446953673
220 0.371057143006718
221 0.370845118513772
222 0.368478538012756
223 0.367439678945027
224 0.366455437591234
225 0.365931703348979
226 0.365246581150922
227 0.365174139266776
228 0.365573720614524
229 0.364007596618707
230 0.364081061136767
231 0.364255513254399
232 0.36309962983619
233 0.362469380226624
234 0.362264321341486
235 0.361689540804164
236 0.361651379188255
237 0.361677203815109
238 0.361769391102169
239 0.361512408237362
240 0.36022246530096
241 0.359611348226255
242 0.359483044890262
243 0.359345260001381
244 0.358447651169047
245 0.3576480685116
246 0.357807133171527
247 0.357127239211777
248 0.356377141834932
249 0.355646501722311
250 0.355308380690887
251 0.355367281708151
252 0.354125944367904
253 0.353927718985912
254 0.353654420829617
255 0.35337014946065
256 0.353041777181068
257 0.353323276114858
258 0.35178360109915
259 0.351543415350827
260 0.351094267210984
261 0.351350988833522
262 0.351586928492555
263 0.351801006764086
264 0.351998810435446
265 0.352336054987943
266 0.352165731133458
267 0.352205172370437
268 0.351837725623134
269 0.352564005684981
270 0.352459914417911
271 0.35252318560122
272 0.351356454349576
273 0.350199291560234
274 0.350596620289307
275 0.35023891743549
276 0.349331854415093
277 0.349126165534346
278 0.349329073446447
279 0.349225674119149
280 0.349569066844876
281 0.348088916209566
282 0.347468511772244
283 0.347061021688501
284 0.346725434763267
285 0.345260534599635
286 0.345884384612521
287 0.344962280505926
288 0.342710910705178
289 0.342485852874913
290 0.342118288026559
291 0.342147546201219
292 0.341691894758987
293 0.341529169753237
294 0.342147288862816
295 0.342474981090834
296 0.34229837618342
297 0.342674995101627
298 0.341730725931395
299 0.341873164434296
300 0.342031488325304
301 0.342291789390851
302 0.342397709018116
303 0.342283493462462
304 0.34025929411806
305 0.340127784738838
306 0.339630992663287
307 0.338680522875203
308 0.337198205873102
309 0.336996518720679
310 0.336251464153845
311 0.335834814339244
312 0.334556127691767
313 0.335081344087111
314 0.335090243533497
315 0.334703020253795
316 0.334983665484362
317 0.334861716988983
318 0.334362064627615
319 0.334921463248193
320 0.334837277114265
321 0.33502933934522
322 0.333831631567481
323 0.333109210340301
324 0.332983229304684
325 0.333046762848186
326 0.333400172844403
327 0.332685157281528
328 0.332667017287712
329 0.332528708833141
330 0.331924293051609
331 0.332246675720677
332 0.33233765416939
333 0.332235933581569
334 0.33264782357222
335 0.331940518090433
336 0.331721387825952
337 0.331272812677991
338 0.331016177434129
339 0.33059589226167
340 0.330495939012565
341 0.330363634508891
342 0.330513943690612
343 0.330018019283277
344 0.329377337739926
345 0.32918939801897
346 0.328658678811569
347 0.328061023410069
348 0.326968735178445
349 0.326451067963568
350 0.326263141318721
351 0.325736992343576
352 0.32553481709495
353 0.325602344189227
354 0.325340281061026
355 0.32512519250114
356 0.324420903974347
357 0.324167120468752
358 0.323846973394247
359 0.323487742617738
360 0.323439844568057
361 0.32358888327316
362 0.323715134919869
363 0.324241804374383
364 0.323621475123696
365 0.323398161294219
366 0.323892897585971
367 0.324173556156245
368 0.323946343774782
369 0.323481155578004
370 0.323261824296669
371 0.322447238757493
372 0.322376244380728
373 0.322934539366631
374 0.322388440943158
375 0.322773910710315
376 0.322095762103112
377 0.3216815951239
378 0.320765419240046
379 0.320521766105014
380 0.32017107891143
381 0.320175096334636
382 0.320282619817573
383 0.319773714269988
384 0.319489454806847
385 0.318812648260105
386 0.318933212788244
387 0.318682847127984
388 0.319034466131389
389 0.319053000570768
390 0.319011313460765
391 0.318762182161609
392 0.31782256447181
393 0.317606204067949
394 0.317570071408268
395 0.317765368593431
396 0.317732435181366
397 0.317476657476216
398 0.317711251694806
399 0.317090666606794
400 0.316533967809405
401 0.316102026354517
402 0.315158825415126
403 0.31469953965375
404 0.314507769073451
405 0.314263416706742
406 0.314471181839346
407 0.31503052724884
408 0.315319689823868
409 0.315342702811124
410 0.315132031649989
411 0.315208584343075
412 0.315222940108305
413 0.315163454674409
414 0.315248115816731
415 0.315364081447072
416 0.315607904389709
417 0.3156833032223
418 0.314550164176612
419 0.314113642904218
420 0.313274280562166
421 0.313259667367971
422 0.312765344007845
423 0.313098400029383
424 0.313003383129784
425 0.313511271221174
426 0.313948786887154
427 0.313900070669908
428 0.314292664544449
429 0.314237312816248
430 0.314700083244353
431 0.313747806218935
432 0.313575769889075
433 0.313920369876926
434 0.314220576630747
435 0.314408716458742
436 0.314144817989559
437 0.313710978363007
438 0.313762540900549
439 0.31401472936799
440 0.314089412981087
441 0.313175401033485
442 0.312820558899073
443 0.312571073656829
444 0.311777028565498
445 0.311641020170908
446 0.31107171905248
447 0.311061422521311
448 0.310759224310271
449 0.310858744610263
450 0.310297739115663
451 0.309802509658791
452 0.310005597435081
453 0.309817075787452
454 0.309931060153077
455 0.30987155855556
456 0.310059527750818
457 0.309638041823967
458 0.310283054266832
459 0.30993752750546
460 0.309696938037335
461 0.309359321500631
462 0.308540828034797
463 0.308610837343914
464 0.308121540914955
465 0.308066982017205
466 0.307960973398302
467 0.307510995964968
468 0.307060589751723
469 0.30711313233432
470 0.307324764409565
471 0.307374160570692
472 0.30652081614592
473 0.306086952844517
474 0.306154281485101
475 0.306075944450165
476 0.306246381643157
477 0.306051860425556
478 0.306143270492168
479 0.305973521125651
480 0.305984724088019
481 0.305852040870808
482 0.305893784893892
483 0.306192437361022
484 0.30630337544009
485 0.306360150883699
486 0.306439317663654
487 0.305864268217289
488 0.306057398740754
489 0.306250941228633
490 0.306532589326687
491 0.306937786589593
492 0.306659799805547
493 0.306466507285366
494 0.30611198810408
495 0.306188519527859
496 0.305946079967354
497 0.305385877459618
498 0.30507769702324
499 0.30546133877554
500 0.305025434347198
501 0.304734345413529
502 0.304908809565427
503 0.304788600717816
504 0.304713129168143
505 0.304826016305539
506 0.304488586919116
507 0.304668151913684
508 0.304594917512635
509 0.304534163864819
510 0.304855427965444
511 0.304549619095526
512 0.303567424339135
513 0.303448279259111
514 0.303083050641596
515 0.303156579678866
516 0.303095119138216
517 0.302781549998952
518 0.302544758812019
519 0.302551836200992
520 0.302663420060167
521 0.302493644938202
522 0.302687402388602
523 0.302716403065714
524 0.302513451799642
525 0.302346676736732
526 0.301595373008051
527 0.301752928246183
528 0.301311380353917
529 0.301473839122313
530 0.301070785049061
531 0.300853518624438
532 0.300543049140269
533 0.30056939881792
534 0.300475164118877
535 0.300053753703425
536 0.300171257982452
537 0.299980949284272
538 0.299817303940664
539 0.299772603821101
540 0.299795245815988
541 0.299533791035739
542 0.299589786617581
543 0.299292633706772
544 0.299254677061125
545 0.299417014044709
546 0.299344898971856
547 0.299464386189295
548 0.299745818766684
549 0.299480567468733
550 0.298925322250859
551 0.29906268780056
552 0.298933642668904
553 0.298399832064454
554 0.298689064958538
555 0.298791169123076
556 0.298193470398931
557 0.297920291188355
558 0.297879373829271
559 0.29784122364023
560 0.297507733289646
561 0.297741628404646
562 0.29754365686279
563 0.297680917139773
564 0.297852331623122
565 0.297722156859258
566 0.2979218248968
567 0.2978771646566
568 0.297844808018237
569 0.297572318849478
570 0.297662638924596
571 0.297878401010902
572 0.298002189474756
573 0.297760481664004
574 0.297330859575402
575 0.296914350073664
576 0.297001526145307
577 0.297246100469016
578 0.297096695005364
579 0.297502616374941
580 0.297617930858205
581 0.297752323144444
582 0.29771364263356
583 0.297973861196499
584 0.297973407981205
585 0.297841082899246
586 0.297727383336264
587 0.297227887105419
588 0.296958809918521
589 0.29698297185528
590 0.297013202758709
591 0.297146744959631
592 0.29680267748209
593 0.296469446761116
594 0.296307114285834
595 0.296364863370114
596 0.296363286452527
597 0.296702366958609
598 0.296444223338311
599 0.296380529023634
600 0.296466720637877
601 0.296310972929354
602 0.296331117619585
603 0.296142052428159
604 0.296126975095478
605 0.295950063673578
606 0.296165813358637
607 0.29626184573712
608 0.296374343529727
609 0.296549932589029
610 0.296573055545564
611 0.296175277009583
612 0.295738752392554
613 0.295783202772308
614 0.295521853282545
615 0.295710179538373
616 0.295604781855245
617 0.295247000195666
618 0.295206560872398
619 0.294944892179482
620 0.294502318744015
621 0.294605830576814
622 0.294849541522511
623 0.294790183310476
624 0.294339885428633
625 0.294008308179289
626 0.293839549518303
627 0.293571946462017
628 0.293478697238348
629 0.293340541910527
630 0.292841723274036
631 0.29276328077133
632 0.292838983042975
633 0.292841662673973
634 0.293023597894353
635 0.292654196050402
636 0.292173824619316
637 0.292196197898489
638 0.292302419275404
639 0.292414180796965
640 0.292700647729931
641 0.292672707163784
642 0.292928320444213
643 0.292969156552649
644 0.293170662675633
645 0.293038673049717
646 0.292714939064885
647 0.293050652073006
648 0.293182650974073
649 0.293131431785776
650 0.292940750954403
651 0.292552960489782
652 0.292107972121551
653 0.292202059127671
654 0.291973168752245
655 0.291830407588922
656 0.291254344972184
657 0.291095163708626
658 0.291064138617003
659 0.290729487464757
660 0.2909542590152
661 0.291020729495541
662 0.291113449029554
663 0.291103863285098
664 0.290774892141285
665 0.290547714933215
666 0.290195054824724
667 0.289898762602896
668 0.289476162284374
669 0.289103172543999
670 0.289324271765078
671 0.289383877063647
672 0.289468568757546
673 0.289075319554485
674 0.28898006839455
675 0.288852751344493
676 0.288728592103961
677 0.288606449553985
678 0.28857584125221
679 0.288844847243424
680 0.289038145730911
681 0.289198440449068
682 0.289362320426442
683 0.289239743781408
684 0.288854732611784
685 0.288888744283518
686 0.288743627698943
687 0.288745732240484
688 0.288589701937939
689 0.288885190050274
690 0.289136176360981
691 0.289275677844809
692 0.289242685839802
693 0.288932609700043
694 0.288817547980279
695 0.288654447426777
696 0.288244919295216
697 0.28821532161021
698 0.288159462897743
699 0.288298015507936
700 0.288251660397471
701 0.288435108678706
702 0.288378367375949
703 0.288725578210697
704 0.288715111209529
705 0.288712260075634
706 0.288345762024402
707 0.287929254640272
708 0.288279501008364
709 0.288264948466813
710 0.28832283868024
711 0.288454003213298
712 0.288482567423956
713 0.288006316741665
714 0.287865620988316
715 0.288243306764291
716 0.288078336209764
717 0.288084635720405
718 0.288152267496498
719 0.287928554178779
720 0.287855110713149
721 0.287785078272656
722 0.287849019135171
723 0.287789182122987
724 0.287781591722969
725 0.287631274382898
726 0.287280701989527
727 0.287152097848477
728 0.286723579786703
729 0.286591798888952
730 0.286430855697896
731 0.286801995138484
732 0.286685208544357
733 0.28685443312857
734 0.28665775113728
735 0.286827186983519
736 0.286930612918899
737 0.287004585462113
738 0.287010351883047
739 0.28711006547941
740 0.287151752422397
741 0.287138191437574
742 0.287373642819355
743 0.287530965139637
744 0.287647923576763
745 0.287948934880008
746 0.287815376470593
747 0.287881365809908
748 0.287949472584568
749 0.287955526362247
750 0.288175719312404
751 0.287963952076353
752 0.287680622753145
753 0.287571942623015
754 0.287622620881869
755 0.287628898104824
756 0.287785139538429
757 0.287601642306183
758 0.287539194207513
759 0.287541310510769
760 0.287522105733906
761 0.287345458124237
762 0.286970907756735
763 0.286913671178105
764 0.287227977985143
765 0.287256455873881
766 0.287382168743103
767 0.287054515789688
768 0.287098213550057
769 0.287323666012697
770 0.287591473376745
771 0.287551068201038
772 0.287347860668963
773 0.287348386105351
774 0.287431289309482
775 0.287029979664018
776 0.287094369912619
777 0.286934496647632
778 0.286841440398165
779 0.286889571761128
780 0.286988904928473
781 0.286760294091017
782 0.286651374055905
783 0.286818767878817
784 0.286583198682591
785 0.286684561170114
786 0.286659944590893
787 0.286603655611108
788 0.286693820959576
789 0.286521754378833
790 0.286348784300821
791 0.286229122111319
792 0.285939986196072
793 0.286154903540078
794 0.285857507518365
795 0.286125299702199
796 0.286267417814422
797 0.286151971623
798 0.286352482486955
799 0.286161099230493
800 0.285902420693819
801 0.286083101877381
802 0.285991896404433
803 0.285739252824049
804 0.285712464251832
805 0.285542742316624
806 0.285286019728742
807 0.285531844500653
808 0.285311504865602
809 0.285252200220054
810 0.285396741177134
811 0.285512318207357
812 0.285598661219843
813 0.285680792063522
814 0.285688653385178
815 0.285336519865128
816 0.285470477808177
817 0.28510257043043
818 0.284923293927245
819 0.284833871419984
820 0.284562774083874
821 0.284575865520324
822 0.284403317580535
823 0.284266215294332
824 0.284472193944354
825 0.284804236969202
826 0.284622862919305
827 0.284705653372406
828 0.284834632861384
829 0.284841834670513
830 0.284909904352817
831 0.284655839546865
832 0.284914386270661
833 0.284683545051598
834 0.284591315444029
835 0.28450478143509
836 0.284279578903551
837 0.284349943674625
838 0.284208626420151
839 0.284298124160221
840 0.284252655107362
841 0.284115538477807
842 0.284260429832408
843 0.284155353761857
844 0.28402714863862
845 0.283554048186982
846 0.283300373991727
847 0.283146373265193
848 0.283248542044306
849 0.283203190510813
850 0.283145494829785
851 0.283146824707816
852 0.282986468630564
853 0.283110924757177
854 0.283273465183646
855 0.283032592419298
856 0.282891283506457
857 0.282721742312654
858 0.282733940107473
859 0.282867140331405
860 0.282617505098939
861 0.282584968108379
862 0.2823343638648
863 0.282431303855338
864 0.282378949160034
865 0.282387960505294
866 0.282185614993881
867 0.282177725220974
868 0.282160858196166
869 0.282080800406969
870 0.281915185155575
871 0.281934790418799
872 0.282024064846573
873 0.281897391596054
874 0.282074053451766
875 0.282087562143764
876 0.281782707301104
877 0.281863200193236
878 0.281900805633919
879 0.281797185072498
880 0.2818972313102
881 0.281914346685682
882 0.281695064344695
883 0.281747077167091
884 0.281705924159653
885 0.281664361305326
886 0.281527212453939
887 0.281458250105183
888 0.281168068264354
889 0.281141706648329
890 0.28108117310533
891 0.281264049964978
892 0.281443136389869
893 0.281555636521533
894 0.281720842908481
895 0.281708562469379
896 0.281579473170773
897 0.281898928576705
898 0.281897885632717
899 0.281874951984209
900 0.281662289187867
901 0.281806802027664
902 0.281709237701722
903 0.28183452915931
904 0.281999505682731
905 0.281941408021892
906 0.281824486857362
907 0.281826768406549
908 0.281690270768456
909 0.281373982069934
910 0.281132312819552
911 0.281000573551698
912 0.281002559841488
913 0.281025405626871
914 0.280732834393591
915 0.280669030287818
916 0.280994544944168
917 0.280752771388243
918 0.280772758005547
919 0.281016910184359
920 0.280641339165167
921 0.280375024008308
922 0.28031605406329
923 0.280399710793644
924 0.280177091302316
925 0.280247977069427
926 0.280317847291452
927 0.280298449679229
928 0.2804579626238
929 0.280379620573367
930 0.280622363510883
931 0.280371691740259
932 0.280461588243783
933 0.280493584898053
934 0.280364077346005
935 0.28045778184987
936 0.280340580791919
937 0.280385679439934
938 0.280441889504284
939 0.280252100992031
940 0.280158190901595
941 0.280293389594301
942 0.280176441082595
943 0.280410861172429
944 0.28044947367998
945 0.280469028444783
946 0.28060517110854
947 0.280327701979324
948 0.280167698442672
949 0.280140892034697
950 0.279905427706676
951 0.28002437029486
952 0.280205262800668
953 0.279824948951314
954 0.27976233281952
955 0.279766047233125
956 0.280065632264879
957 0.279973056091753
958 0.279922045964623
959 0.279992974637183
960 0.280315719790032
961 0.280308232192824
962 0.280286119634865
963 0.280199728571645
964 0.280116844891926
965 0.280218334748781
966 0.280222357816276
967 0.280549987100131
968 0.280549482708347
969 0.280442042587216
970 0.280232611804591
971 0.279949514955301
972 0.280085051501227
973 0.280191682659929
974 0.280349660193151
975 0.280455281964544
976 0.280177388975941
977 0.280352719543319
978 0.280221566594257
979 0.28036923239613
980 0.28039388324271
981 0.280274039765673
982 0.280240557054698
983 0.279996894998003
984 0.27981412315737
985 0.279734147140765
986 0.27978980214913
987 0.279581431827717
988 0.279669226928283
989 0.279762771997673
990 0.279880515564218
991 0.279779575812858
992 0.279755668772421
993 0.279899165182974
994 0.27973275789488
995 0.279759261587448
996 0.279863125541115
997 0.279836504249274
998 0.279895481602248
999 0.279961826006102
1000 0.279984565479981
};
\addlegendentry{kernel herding}
\addplot [semithick, color1]
table {%
1 1.20399022168974
2 1.14090646501583
3 1.10915078471357
4 1.07064256551802
5 1.01917773305795
6 0.989260572917173
7 0.972400808770127
8 0.955576213887253
9 0.936050080474437
10 0.922671529067111
11 0.903319732822067
12 0.888573175151509
13 0.876682790139927
14 0.860163798148562
15 0.845967430491757
16 0.831041725167685
17 0.820949197549775
18 0.802408157352011
19 0.79113793655615
20 0.783230371738369
21 0.777103850149684
22 0.77189148860365
23 0.765446793667881
24 0.756136404310473
25 0.741555518775331
26 0.733237503418243
27 0.725832790153625
28 0.718305587855328
29 0.710338043962801
30 0.698554129429809
31 0.687295671718555
32 0.682781516253149
33 0.673270053081036
34 0.668056428931729
35 0.662027895656589
36 0.654143256374506
37 0.64660669853402
38 0.638259029700049
39 0.634484395413584
40 0.629098495295001
41 0.623125028388971
42 0.617396732045169
43 0.613507171226373
44 0.60974029953949
45 0.60555949834695
46 0.599295707190386
47 0.592978217851217
48 0.588630862736563
49 0.584625519794053
50 0.581877430320903
51 0.579761672890565
52 0.577107723381679
53 0.571627874648758
54 0.569005010269653
55 0.567032419104294
56 0.563229673652036
57 0.560752761114636
58 0.552234936568151
59 0.549557129872629
60 0.543779994291627
61 0.541388699312342
62 0.536097997062375
63 0.534432256989502
64 0.532759390115891
65 0.531746385484689
66 0.527997214107621
67 0.526355879388026
68 0.524228386885178
69 0.521121720653128
70 0.51500003406439
71 0.51034897214454
72 0.506090034984404
73 0.505812895983418
74 0.501926010524015
75 0.50018202791324
76 0.498677706171035
77 0.495519223489436
78 0.493805186643803
79 0.4933472818133
80 0.491079192561362
81 0.488336313155552
82 0.486360414830005
83 0.482992514505574
84 0.478426780549554
85 0.476362812982958
86 0.474853133132904
87 0.471221207096123
88 0.470122646687129
89 0.469538637366835
90 0.467517829314259
91 0.460752363946301
92 0.459286489343624
93 0.459034653310405
94 0.456446765402985
95 0.452016380771577
96 0.451637112990047
97 0.45116221912195
98 0.449445883895539
99 0.448532691816418
100 0.44540249683134
101 0.440674343514599
102 0.438892792253782
103 0.436373315212852
104 0.435188610754329
105 0.435446052665543
106 0.433843811062778
107 0.433447204070426
108 0.432830740308939
109 0.430970551816793
110 0.428134339537092
111 0.426585318835997
112 0.426703318491715
113 0.425692076948526
114 0.424762486051603
115 0.424393866141729
116 0.422537146577712
117 0.42012631596749
118 0.419662564740831
119 0.419142502539115
120 0.417509630940707
121 0.416088104951137
122 0.415376210131291
123 0.412513736133979
124 0.410358017250544
125 0.407738535270144
126 0.40826819179324
127 0.407014877719814
128 0.405917881552186
129 0.40488430601728
130 0.402808126606942
131 0.401648207996401
132 0.401087275305972
133 0.400545348733132
134 0.399609550943337
135 0.3981623569177
136 0.396671057792332
137 0.396971743214453
138 0.394140458457207
139 0.390802154004976
140 0.389052569976434
141 0.389278357592439
142 0.389439361109335
143 0.389325244018554
144 0.388334371924323
145 0.388304959049585
146 0.38776104466814
147 0.387197773437354
148 0.385791378457984
149 0.384349233578562
150 0.381611239315349
151 0.379283305121963
152 0.377990778105505
153 0.377311193834496
154 0.377157668693398
155 0.375299917966424
156 0.374621166843696
157 0.373933707745951
158 0.372792479052987
159 0.37257950563541
160 0.37104520789389
161 0.37049770947937
162 0.368378687366503
163 0.367930078747966
164 0.366787856365513
165 0.366747175543481
166 0.366450455054576
167 0.364927873462806
168 0.363660415652894
169 0.363425232144505
170 0.362334418386636
171 0.362246420222138
172 0.361809846862443
173 0.361289702085473
174 0.361267392312488
175 0.360719766608224
176 0.359395882268304
177 0.358160410207222
178 0.356930420592152
179 0.354904176180691
180 0.353266016630612
181 0.351342216121138
182 0.350407274255355
183 0.350074763706257
184 0.350335141823189
185 0.350546669450269
186 0.349876867415175
187 0.349372020544906
188 0.348843459513243
189 0.34876647794071
190 0.348503456245012
191 0.348108274729432
192 0.347512012867733
193 0.347415638244764
194 0.347948855314006
195 0.346966358513004
196 0.346459880416506
197 0.346290418208828
198 0.345797403252831
199 0.344744860530125
200 0.344040863168273
201 0.344227474238413
202 0.343631635649559
203 0.343541454758788
204 0.342127576872262
205 0.341858987285543
206 0.340310651560334
207 0.339271542201516
208 0.338774802223541
209 0.337551954566563
210 0.337845864927916
211 0.336923250568813
212 0.337047992454443
213 0.336067905237608
214 0.336145618117203
215 0.336593927511352
216 0.336545371702934
217 0.335581652176932
218 0.335352567767244
219 0.334384066341334
220 0.333929447368629
221 0.334081859974943
222 0.333837301109391
223 0.333210544925333
224 0.33290551454118
225 0.333203427403678
226 0.332917727432527
227 0.333337487360893
228 0.333525900798674
229 0.33260383575906
230 0.331667485173059
231 0.33073230513572
232 0.330598393556026
233 0.329990025388512
234 0.330244568925453
235 0.32993249138571
236 0.330060704015819
237 0.330616696423889
238 0.330047520169537
239 0.329870741389578
240 0.329520467816104
241 0.329862217651814
242 0.330386077245151
243 0.33027361805054
244 0.331049061526235
245 0.330507362900279
246 0.328792240842831
247 0.328152000412788
248 0.328007462701999
249 0.326031465449617
250 0.325259797448984
251 0.324389146029091
252 0.323793492771669
253 0.323277407987686
254 0.322579341618506
255 0.322470873559462
256 0.322361890013455
257 0.321227481159197
258 0.321038055231914
259 0.318864082646871
260 0.318143119324143
261 0.317491039773099
262 0.316458338228168
263 0.315874993325571
264 0.31593324954332
265 0.315353510411956
266 0.314993369486553
267 0.313201557743609
268 0.313472646793007
269 0.313002417133982
270 0.312365584346238
271 0.311800709077323
272 0.311901050348816
273 0.311373766771526
274 0.311276362126211
275 0.311171155787142
276 0.310781406168208
277 0.310673847244611
278 0.310118591015306
279 0.309329304780956
280 0.308597182045872
281 0.308433557388153
282 0.308513804363387
283 0.308360798114044
284 0.309003447146489
285 0.308931589344785
286 0.307562676331377
287 0.306973303608839
288 0.307001472941849
289 0.306852916610302
290 0.306011218200701
291 0.305789533352606
292 0.306077851223251
293 0.305693148104531
294 0.305953241446873
295 0.305201181267534
296 0.304683732026464
297 0.303948453781491
298 0.304063074098537
299 0.303268602964843
300 0.303088858200042
301 0.303174458416122
302 0.302652183325986
303 0.302347328170594
304 0.302330497913901
305 0.301877011498333
306 0.301952097526391
307 0.301795346866
308 0.301341394461867
309 0.300794772213818
310 0.300693377510231
311 0.300158180527893
312 0.299625254157985
313 0.29949959024399
314 0.299198609679859
315 0.299711020411661
316 0.30019412204898
317 0.300358967062339
318 0.299530791786924
319 0.299447252350482
320 0.299253766813195
321 0.2984809214598
322 0.297541720991904
323 0.297703824844266
324 0.297313403500585
325 0.296232088186248
326 0.294868998990974
327 0.294486003252841
328 0.294489319839626
329 0.294127227510704
330 0.293382204283236
331 0.293076032884795
332 0.292929210716297
333 0.29308413540311
334 0.292596630244436
335 0.291897601142871
336 0.291219992007281
337 0.291471535493406
338 0.29166446274955
339 0.291333157759801
340 0.291393564006786
341 0.29108334430129
342 0.290713362192315
343 0.289602140642961
344 0.28982431460658
345 0.289545271239259
346 0.289223930074885
347 0.289192975429849
348 0.288735684019392
349 0.288317129304635
350 0.288497542520273
351 0.287952132297775
352 0.287659758863818
353 0.28805722088835
354 0.288388733518391
355 0.287677633579321
356 0.288120065290078
357 0.28816710517054
358 0.288623282377948
359 0.288553411460739
360 0.288698967080989
361 0.288727922065944
362 0.288517553807718
363 0.288145439979394
364 0.28754650764361
365 0.286916965291635
366 0.28674899880364
367 0.287061406173036
368 0.287109088985101
369 0.28699142597876
370 0.286781077983905
371 0.286928877781257
372 0.287153884117827
373 0.287244843100309
374 0.286372639491243
375 0.286296379988866
376 0.285823916746611
377 0.285430490362758
378 0.285394605087783
379 0.285509749331474
380 0.285763272246274
381 0.285939014167695
382 0.285712715958231
383 0.28489730718694
384 0.284295564399069
385 0.284165740776553
386 0.284009277312918
387 0.283319714162221
388 0.283210246052035
389 0.283047939328723
390 0.28269515301917
391 0.283253961105737
392 0.282790090691104
393 0.282815063683918
394 0.283498252017136
395 0.283288364691312
396 0.283126651296433
397 0.283380295399198
398 0.28305610856339
399 0.282737213682699
400 0.28255790119531
401 0.28213782014352
402 0.281347861792167
403 0.281036050127079
404 0.280870191819097
405 0.280833535168707
406 0.281023006565987
407 0.280773251138086
408 0.280057906288262
409 0.279918445293972
410 0.279198614036782
411 0.278714475639688
412 0.278391816091569
413 0.278095409661182
414 0.277769658049272
415 0.277224461845839
416 0.276969839903658
417 0.276260105985158
418 0.276523306363075
419 0.27690469343351
420 0.277100246685586
421 0.276862307319656
422 0.276529210019639
423 0.276778249339748
424 0.276736912195053
425 0.276661052843923
426 0.276811174540185
427 0.277256848105015
428 0.276899831860955
429 0.276334172648112
430 0.276022681777551
431 0.275798998965108
432 0.275915574833003
433 0.275859785604066
434 0.276008180444012
435 0.276181661080497
436 0.275908330610496
437 0.275482388927198
438 0.275009299268278
439 0.275153186766007
440 0.27550152375255
441 0.27510085443778
442 0.27564067029303
443 0.275616112836392
444 0.275597623824981
445 0.275679188163024
446 0.275267505428829
447 0.275269577767912
448 0.274594534855131
449 0.273909047021383
450 0.273370610775464
451 0.27332667739147
452 0.27336543904757
453 0.273468778816405
454 0.273274191189066
455 0.272942368654227
456 0.27254804260909
457 0.272223113566588
458 0.272198609577954
459 0.272371967556538
460 0.27246030111593
461 0.272514627137621
462 0.271989317961656
463 0.271255202523986
464 0.271106905742713
465 0.270477409474198
466 0.269727292582062
467 0.269255107083059
468 0.268876044643397
469 0.268856610298641
470 0.269256563736487
471 0.269099666446341
472 0.26909487047036
473 0.268212447041006
474 0.267783247147914
475 0.267615348079764
476 0.267383689924842
477 0.267179471950147
478 0.267145416456967
479 0.267294804285731
480 0.267307817218908
481 0.266827336477746
482 0.266755948759618
483 0.266834302094165
484 0.266821250033607
485 0.2669613864953
486 0.267006693774557
487 0.267732818110529
488 0.267489800918777
489 0.267729889916411
490 0.267538903929367
491 0.267636731398067
492 0.267876591435226
493 0.268031065235078
494 0.267537925771371
495 0.267634980295225
496 0.267054246706066
497 0.267136062925773
498 0.267245037063114
499 0.267108820965735
500 0.266786719744829
501 0.266446896252312
502 0.26616945220945
503 0.265547098457367
504 0.265435304801252
505 0.265477679716194
506 0.265212410742471
507 0.265514844999078
508 0.265806289418595
509 0.265994171903889
510 0.265732113967941
511 0.265809467669284
512 0.265551528827655
513 0.265510504476321
514 0.265533989833897
515 0.265261549449412
516 0.265123740161434
517 0.264716341966749
518 0.264443980795931
519 0.264102117726769
520 0.263828895594415
521 0.263926544029491
522 0.263784859765728
523 0.263626847222134
524 0.263952760849931
525 0.264217775831564
526 0.264210526286535
527 0.263736322031002
528 0.263603665498158
529 0.263879109988699
530 0.263999603793055
531 0.263889569357228
532 0.263144153578484
533 0.262801018428684
534 0.262609808525406
535 0.262644636777325
536 0.262291655001439
537 0.262560631715029
538 0.262485480420447
539 0.262194426701707
540 0.261755580194445
541 0.261870416476083
542 0.261809391916848
543 0.261981160946621
544 0.262023177386381
545 0.261626079911754
546 0.261726428192803
547 0.26172040861481
548 0.261335089872312
549 0.261522309814805
550 0.261629171119694
551 0.261747273445326
552 0.261829207587894
553 0.261597989443082
554 0.261702583674628
555 0.261600869729556
556 0.261801027439563
557 0.261878558343647
558 0.261941417031186
559 0.261852373801275
560 0.261701027572837
561 0.261608822675174
562 0.261471383582235
563 0.261292111783596
564 0.261321901925128
565 0.261508790236758
566 0.261791815711352
567 0.261511784245663
568 0.261370731930097
569 0.260903461644
570 0.260766077453958
571 0.260745332211599
572 0.260174568171211
573 0.260146875898341
574 0.259946339608719
575 0.259828061633237
576 0.259445869559932
577 0.259145778229191
578 0.259347681683781
579 0.259208857501115
580 0.258870736798752
581 0.259066328652323
582 0.25888982219697
583 0.258973484295295
584 0.259375303745059
585 0.258954889657698
586 0.258869366539289
587 0.258830584531279
588 0.258706689786848
589 0.258123459867421
590 0.257920548640706
591 0.257639786364546
592 0.257600383122052
593 0.257590904646047
594 0.257758609311744
595 0.257743549305407
596 0.257769736358497
597 0.258004874705959
598 0.257535723539393
599 0.257252415010435
600 0.257023906638788
601 0.257007813023446
602 0.256552038689237
603 0.256508827512089
604 0.25631683158162
605 0.256413510039979
606 0.256439525919547
607 0.256584894685535
608 0.256707721697553
609 0.256662000707016
610 0.256455102145173
611 0.256027399215383
612 0.255730496078114
613 0.255812569153803
614 0.255777131498891
615 0.255698609875313
616 0.255464611746653
617 0.255318240674874
618 0.255449134424023
619 0.255132476467538
620 0.255093868234807
621 0.255261536330672
622 0.255125692909069
623 0.255220898810565
624 0.254854570316473
625 0.255104097745941
626 0.2552351342102
627 0.25524703554848
628 0.255039435978193
629 0.254926014801635
630 0.255035657375173
631 0.25511757989553
632 0.255590677813192
633 0.255665641266703
634 0.255705211832563
635 0.255559963787747
636 0.255153717411861
637 0.255074566455159
638 0.255294636954001
639 0.255038102057685
640 0.255040615062864
641 0.254568940615067
642 0.254808682438373
643 0.25436732099071
644 0.254283098855224
645 0.254118394923767
646 0.254038529781893
647 0.254075107846742
648 0.254170397582464
649 0.254096468259348
650 0.253708892553467
651 0.253721511523035
652 0.253998908404936
653 0.253836098193112
654 0.25380536094578
655 0.253956695441905
656 0.253910708351392
657 0.253741013728621
658 0.253820400541435
659 0.253623251882914
660 0.253782162618821
661 0.253715083033054
662 0.25368710162097
663 0.253504398389612
664 0.253306436910478
665 0.25313759993803
666 0.252994230623278
667 0.253002583851776
668 0.253158797321848
669 0.253312577994454
670 0.253160101543337
671 0.252865662141201
672 0.252630489905803
673 0.252627631427603
674 0.252679016430996
675 0.252888007120691
676 0.252576323068768
677 0.25251350929916
678 0.252533175520873
679 0.252443176501597
680 0.252100370194716
681 0.252410316136642
682 0.252321310136066
683 0.252394702594312
684 0.252137203049975
685 0.252090518311878
686 0.251704763116616
687 0.25109586203383
688 0.251328693859308
689 0.251477668011214
690 0.251729762551456
691 0.251834568438412
692 0.251902777869913
693 0.251716307900885
694 0.251969053836577
695 0.252334064901528
696 0.252441976918871
697 0.251990672451005
698 0.251752043778295
699 0.251695354265808
700 0.25120163423599
701 0.251006813626252
702 0.251006872437566
703 0.251242626679985
704 0.251002266042933
705 0.251141687008106
706 0.251159934871172
707 0.251147198353129
708 0.251314272166354
709 0.251269280469329
710 0.25175803622034
711 0.251801238043006
712 0.25164899427841
713 0.251678774718019
714 0.251565977615287
715 0.251496324506648
716 0.251552333555208
717 0.251511264954451
718 0.251501579377289
719 0.251004862167697
720 0.250981175795577
721 0.250944080723804
722 0.250809317370178
723 0.250700436237127
724 0.250408242200101
725 0.250442381881267
726 0.250276595729752
727 0.250199337647069
728 0.249993040371898
729 0.249983016109395
730 0.250074340884888
731 0.250072731255234
732 0.249688478625179
733 0.25001476643101
734 0.249902485569367
735 0.249621654954646
736 0.249595882188786
737 0.24940421706459
738 0.249425801200652
739 0.249500547388104
740 0.249378921610697
741 0.249480228053536
742 0.249883823655263
743 0.249763642028388
744 0.249764754915566
745 0.24992823088411
746 0.250207761706681
747 0.250328917866748
748 0.250215002049803
749 0.249876648262502
750 0.249806490213661
751 0.249988897152227
752 0.249921177465656
753 0.250148634070857
754 0.250136211474991
755 0.250098659210741
756 0.249958187705899
757 0.249810692425899
758 0.249648665539031
759 0.249470310459516
760 0.249207905268966
761 0.24916087537886
762 0.249235107250559
763 0.249190614312556
764 0.249303036877651
765 0.249454185560192
766 0.24933999546933
767 0.249168937532414
768 0.249138058324732
769 0.249124280625122
770 0.248714724085425
771 0.248584930973912
772 0.248759431291164
773 0.248525698703843
774 0.24853283019326
775 0.248708886269776
776 0.248760494517066
777 0.248865798646035
778 0.24904318871445
779 0.248978455837615
780 0.248725689328356
781 0.248413374563486
782 0.248634866157003
783 0.248517579564388
784 0.248377354237901
785 0.248291864446902
786 0.248342362039272
787 0.248293573239368
788 0.248037440374746
789 0.247745204467242
790 0.247683971363295
791 0.247521298983787
792 0.2473816900214
793 0.247157779559818
794 0.247065423811711
795 0.247081509369818
796 0.246967632572946
797 0.246727527624858
798 0.246494738839577
799 0.246674497708448
800 0.246536880512439
801 0.246682642769817
802 0.246551362551461
803 0.2465353895387
804 0.246547495552631
805 0.246561600595013
806 0.246746066046734
807 0.2466477005393
808 0.246927492767235
809 0.246836170219947
810 0.246976189376948
811 0.246996737633426
812 0.246710475667604
813 0.246574105340849
814 0.246286962221358
815 0.246055419358627
816 0.245963667148594
817 0.245960038196171
818 0.245884606238533
819 0.245908025304321
820 0.245909616379682
821 0.24586961250383
822 0.245913694348686
823 0.246113694672061
824 0.245759254749618
825 0.245595719958804
826 0.245699391775077
827 0.245646771222498
828 0.24578496960431
829 0.245778319508296
830 0.245779668147609
831 0.24559867566829
832 0.245478232472047
833 0.245046759869662
834 0.245206273717584
835 0.24524650755668
836 0.245336737111831
837 0.245217653772305
838 0.245358758140397
839 0.245290646026824
840 0.245376561842394
841 0.245585406916116
842 0.245281030407492
843 0.245254495414156
844 0.245019146998514
845 0.245157215090156
846 0.244976345376792
847 0.245075187049061
848 0.245164896721932
849 0.245270178807928
850 0.244937575934379
851 0.244962740013246
852 0.244826501576413
853 0.244741214733107
854 0.244723592508251
855 0.244489139157538
856 0.244443072030629
857 0.244638087084187
858 0.24438897045886
859 0.244315437851465
860 0.244326254645134
861 0.244146993484003
862 0.244130567009198
863 0.244113391605286
864 0.244184885691565
865 0.243997016586542
866 0.243825623320961
867 0.243679199123644
868 0.243667933155507
869 0.243282170454072
870 0.243009291995932
871 0.242845047006628
872 0.242858106532964
873 0.242867868399578
874 0.2428590690905
875 0.242839488682061
876 0.242826985563115
877 0.242813854448475
878 0.24290570839811
879 0.243103331339298
880 0.24299979395306
881 0.242948077572409
882 0.243009355096823
883 0.243099247707889
884 0.243187369905145
885 0.243300278156626
886 0.243198693877605
887 0.243304328260015
888 0.243074995961587
889 0.243011889263247
890 0.242611526981966
891 0.242551309883188
892 0.24276345622954
893 0.242715095215188
894 0.242568070945153
895 0.242709952917112
896 0.242815234193366
897 0.24273892335403
898 0.242580059631017
899 0.242664253514199
900 0.242386830947068
901 0.24230921865697
902 0.242383153389421
903 0.242480405827436
904 0.242546832651899
905 0.242324200036828
906 0.242364461715278
907 0.242281388353192
908 0.242125585611217
909 0.24212881110116
910 0.242204751598029
911 0.242201117533191
912 0.242117207885446
913 0.242124546911764
914 0.242035318577653
915 0.242136528004817
916 0.242082688182505
917 0.242140667357922
918 0.24203030736135
919 0.242157214909451
920 0.242122997841857
921 0.24215491809682
922 0.242283212741538
923 0.242147615590953
924 0.242305081024255
925 0.242263337499106
926 0.242289362283775
927 0.24216707422394
928 0.241895730039775
929 0.241781657112817
930 0.241742202855089
931 0.24202366043745
932 0.241965953984859
933 0.241769290815188
934 0.241846066801353
935 0.241934374487667
936 0.24202555989636
937 0.242195040061317
938 0.242126410720887
939 0.242010607673375
940 0.241982841163278
941 0.242170248687426
942 0.242341534399187
943 0.242371498327784
944 0.242478693523622
945 0.242226704545517
946 0.242170797454883
947 0.242058703813768
948 0.242032283312792
949 0.242000632232655
950 0.24176709582969
951 0.241706334975869
952 0.241707588402452
953 0.241705187746692
954 0.241523878101136
955 0.241687253776268
956 0.241659993023527
957 0.241581636592931
958 0.241572224612346
959 0.241559253563979
960 0.241599923882559
961 0.241561310203647
962 0.241612536422748
963 0.241611632241355
964 0.241461874141986
965 0.241567646551582
966 0.241590593476416
967 0.241653725548943
968 0.241520279197664
969 0.241383850188997
970 0.241400503688717
971 0.241446570923713
972 0.241477000234809
973 0.241671102874885
974 0.241777150786972
975 0.241640233092095
976 0.241386364024641
977 0.241330532807942
978 0.241539246590606
979 0.241398556014808
980 0.241356862157201
981 0.241502065146197
982 0.241542704519908
983 0.241409781928449
984 0.241347113027555
985 0.24151722275438
986 0.241376651156516
987 0.241320400448932
988 0.241290830209068
989 0.241431290960875
990 0.241362210451841
991 0.241111741605888
992 0.241116553995278
993 0.241057375618172
994 0.241208990337718
995 0.241137222793425
996 0.240930906437759
997 0.240906439460885
998 0.240820950588322
999 0.240810210459821
1000 0.240870740716645
};
\addlegendentry{continuous herded Gibbs sampling}
\addplot [semithick, color2]
table {%
1 1.33901207384727
2 1.31524902603361
3 1.29919739673125
4 1.28337632782679
5 1.26959719663405
6 1.26076163994118
7 1.25134574023697
8 1.24531829136827
9 1.23918293755125
10 1.23449679418426
11 1.22693494146886
12 1.21890955511269
13 1.21457509652626
14 1.20925189319227
15 1.20360876355518
16 1.1992239148962
17 1.1962014550164
18 1.1924657048719
19 1.18854349293217
20 1.18432556826158
21 1.18068262308438
22 1.17716795939805
23 1.17329728335662
24 1.17083836509171
25 1.17023735453325
26 1.16825724674308
27 1.16675942805528
28 1.16458700346673
29 1.16253026310772
30 1.16036321492335
31 1.15716774470778
32 1.15620083910472
33 1.15421158343435
34 1.15266743397823
35 1.15101772128367
36 1.1480018161893
37 1.14583515576516
38 1.14299556768915
39 1.14125483053071
40 1.1401329787299
41 1.13900394714432
42 1.13712438758599
43 1.13637556237991
44 1.13445327522502
45 1.13230135866654
46 1.13115339260227
47 1.12975751716345
48 1.12784302391487
49 1.1267286986067
50 1.12588395336474
51 1.12384195064851
52 1.12204869975617
53 1.12080767309457
54 1.11897941662073
55 1.11754417434585
56 1.11537284486026
57 1.11451074416215
58 1.1136364592786
59 1.11281989541272
60 1.11194636895708
61 1.11042673498289
62 1.10855117029676
63 1.10783180326083
64 1.10602649560373
65 1.10489992299936
66 1.10299933385944
67 1.10196747314406
68 1.1009404426151
69 1.09968521109071
70 1.09843342690417
71 1.09747345591675
72 1.09596138811851
73 1.09504144250953
74 1.09417007626609
75 1.09280456198853
76 1.09189521276666
77 1.09082370069471
78 1.08966551784648
79 1.0891804661985
80 1.08854139876279
81 1.08740306097893
82 1.08666883369037
83 1.08516696264926
84 1.08400407028091
85 1.08309417249856
86 1.08229626446357
87 1.08091342088335
88 1.07957116375053
89 1.0787969101486
90 1.07810487553436
91 1.07722087932165
92 1.07668480331207
93 1.07576596613614
94 1.07474099079029
95 1.07387511908279
96 1.0730458729732
97 1.07231617644514
98 1.07079548264092
99 1.07004512383366
100 1.0692395726553
101 1.06843006005314
102 1.06789882082375
103 1.06734869067169
104 1.06643453113368
105 1.06551466154941
106 1.06462533659403
107 1.06355004192951
108 1.06241934760059
109 1.06165255155855
110 1.06070330498963
111 1.05980544431783
112 1.05904700656931
113 1.05794401708095
114 1.05726625770699
115 1.05655991855688
116 1.05517671670577
117 1.05447271789877
118 1.05315371688788
119 1.05194697384775
120 1.0510056167158
121 1.04993779944307
122 1.04906473135564
123 1.04749332696204
124 1.04630151623299
125 1.04523946272457
126 1.04418054592465
127 1.04275836548356
128 1.04171873022775
129 1.04001579413461
130 1.03909059375092
131 1.03790251916465
132 1.03683519494201
133 1.03562575753157
134 1.03445581234855
135 1.03320099059793
136 1.03212441124814
137 1.03088883846776
138 1.02996985523209
139 1.0284766335604
140 1.02740985220007
141 1.02620175717105
142 1.02531632670324
143 1.02389703079138
144 1.02319044676951
145 1.02190723616072
146 1.02070546790359
147 1.01991018497968
148 1.01897107371605
149 1.0180927516505
150 1.01689404863778
151 1.01579971794633
152 1.01443221205461
153 1.01343354407593
154 1.01245533500821
155 1.01130498321754
156 1.01036459919032
157 1.00919122603865
158 1.00826776953196
159 1.0070986951902
160 1.00642864088864
161 1.00558018766439
162 1.00468389423807
163 1.0037890855957
164 1.00282905299522
165 1.00212123145865
166 1.00091306840686
167 0.999603414230091
168 0.998855738400523
169 0.998084836938844
170 0.996728615687721
171 0.995944302650551
172 0.995415040773644
173 0.994534772924173
174 0.993704627945211
175 0.992867663495675
176 0.991970716247401
177 0.991061868287381
178 0.990228935918636
179 0.989591927643082
180 0.988970243062323
181 0.988179832708622
182 0.987275751103561
183 0.986255480963052
184 0.985523408481911
185 0.984573848123214
186 0.983480087006262
187 0.982643194508222
188 0.981575886203353
189 0.980391660239845
190 0.979465705940944
191 0.978492114366688
192 0.97772484892132
193 0.976863577486557
194 0.975891303355006
195 0.975010060507927
196 0.97412133806256
197 0.973207633463788
198 0.971891006248658
199 0.9708675833507
200 0.969786642981197
201 0.96882516466646
202 0.967762450218879
203 0.966907217997154
204 0.965901558444401
205 0.964687730246715
206 0.963684266576944
207 0.962641006202348
208 0.961686678201245
209 0.960530262219448
210 0.95957547756512
211 0.958336756922726
212 0.957124025864991
213 0.956149926350705
214 0.955290157192289
215 0.954394630049805
216 0.953327679628037
217 0.952235368051286
218 0.951213906802626
219 0.949919230636999
220 0.948729705489858
221 0.94740952850024
222 0.946067448136753
223 0.944785171093156
224 0.943886270789834
225 0.942898852640404
226 0.941656994159264
227 0.940806551432079
228 0.939672547594136
229 0.938710981546414
230 0.937633981479551
231 0.936189479634518
232 0.93516106149106
233 0.934217656826188
234 0.93306402045769
235 0.932182043883014
236 0.931116045127146
237 0.930332296541214
238 0.929104718911662
239 0.928194296610505
240 0.926951322305855
241 0.9257938022884
242 0.924563411925616
243 0.92361905780742
244 0.922593610375076
245 0.921590463776775
246 0.920805092949805
247 0.919642668844158
248 0.918856926682821
249 0.917984114258119
250 0.916784359448466
251 0.915719509012155
252 0.914817088473529
253 0.91403953880122
254 0.913015262401757
255 0.911829872122592
256 0.910983367979103
257 0.90992238993558
258 0.909164626573691
259 0.908241214214426
260 0.907008936374151
261 0.905903083128931
262 0.904980406066993
263 0.904111969046362
264 0.902903554420097
265 0.902302421060824
266 0.901282222760167
267 0.900371624616455
268 0.899406435399848
269 0.898504518861375
270 0.897384485364059
271 0.89664317881243
272 0.895845738141272
273 0.894738775516281
274 0.893783533252738
275 0.892517956083118
276 0.891257987428835
277 0.890381408501222
278 0.889345779587605
279 0.888448291357577
280 0.887400304481373
281 0.886517328815888
282 0.885559901481195
283 0.884678100721124
284 0.883742165018284
285 0.882873000943
286 0.882113472562578
287 0.881372310793299
288 0.88036220398426
289 0.879366970530392
290 0.878569111351885
291 0.877406734265931
292 0.876414041881065
293 0.875697032428644
294 0.874901437753153
295 0.874065070010357
296 0.873128841715263
297 0.872312581203802
298 0.871257507052833
299 0.870315530167566
300 0.86951856464054
301 0.868500617072449
302 0.867642251820431
303 0.866831064793503
304 0.866057025160469
305 0.865109516647443
306 0.864324549582954
307 0.863388534900906
308 0.862723170432306
309 0.861707976101695
310 0.86083491175414
311 0.859842547055931
312 0.859201983925912
313 0.858318001958638
314 0.857542002841008
315 0.856703285257714
316 0.855808048584103
317 0.854859404044466
318 0.853982183582207
319 0.853402995251696
320 0.852489413732739
321 0.851938856409112
322 0.851099265556377
323 0.850143844105676
324 0.849438819376924
325 0.848820168833353
326 0.847895307054538
327 0.847134487575493
328 0.846479400143805
329 0.845757436917939
330 0.84536487934704
331 0.844770983902254
332 0.843890780413011
333 0.843349843852237
334 0.842608363507369
335 0.841849081086765
336 0.841076713128069
337 0.84044041526404
338 0.839616359657379
339 0.839060183759666
340 0.838301634705283
341 0.837690243018785
342 0.83691920770394
343 0.836239588561936
344 0.835425618252682
345 0.83451395553047
346 0.833727069493502
347 0.833294888382663
348 0.832716585960712
349 0.831819144993052
350 0.831159695837029
351 0.830443029542237
352 0.829761462001178
353 0.829031760150382
354 0.828285106530593
355 0.827465108343288
356 0.826670143181643
357 0.825705757922067
358 0.825091622131815
359 0.824454337209839
360 0.82373917880331
361 0.822850039364687
362 0.822131683874132
363 0.821416498990291
364 0.82071121833591
365 0.819711871747688
366 0.818811485366172
367 0.818253050449711
368 0.817592219302893
369 0.816833456580746
370 0.816161063051878
371 0.815085863576501
372 0.814605997631463
373 0.813806015627307
374 0.812874533743908
375 0.812044665975841
376 0.811271432337701
377 0.810297145993329
378 0.809501966998068
379 0.80860737341675
380 0.807975526945907
381 0.807307643136245
382 0.806219642996093
383 0.805461863036565
384 0.804680156124101
385 0.803973134116573
386 0.803168687217315
387 0.802264970614769
388 0.801368564812139
389 0.800541170572348
390 0.79949831426167
391 0.798491714435191
392 0.797755440127129
393 0.796767204667161
394 0.795915195083697
395 0.794967896446209
396 0.794089251659398
397 0.793322604544118
398 0.792340483383869
399 0.791415212862025
400 0.790413129964519
401 0.78958039250846
402 0.788689824845915
403 0.7879218302395
404 0.786959767524549
405 0.785953997039868
406 0.784845899154782
407 0.78379544571745
408 0.782785859034511
409 0.781858785673745
410 0.780818664918593
411 0.779514728166525
412 0.778213327367549
413 0.777121902847338
414 0.775924421551385
415 0.774705356633711
416 0.773459202221219
417 0.772421590772002
418 0.771118671717835
419 0.769692038911586
420 0.768435320576459
421 0.767351633051304
422 0.766044751296825
423 0.764717823049398
424 0.763288192943224
425 0.762067572926959
426 0.760818525093398
427 0.759699583122389
428 0.758305390447644
429 0.756861534694069
430 0.755395186198062
431 0.753957887147611
432 0.752591650570158
433 0.751273014579195
434 0.750042653294357
435 0.748848640764159
436 0.747417487764125
437 0.746236663668296
438 0.744838525298876
439 0.74362122776048
440 0.74225133173962
441 0.741159795282806
442 0.739934830596283
443 0.738605038665981
444 0.737399390211462
445 0.736160742590881
446 0.735183501063428
447 0.73391215690919
448 0.73264871614048
449 0.731470718338123
450 0.730340177272494
451 0.729339176547167
452 0.728304310053579
453 0.727223515521452
454 0.726085955469298
455 0.724961698271268
456 0.723793918166617
457 0.72273615247638
458 0.721613493792627
459 0.720552433875964
460 0.719275734121759
461 0.718231860084292
462 0.717232142629387
463 0.716217166823968
464 0.715283805202144
465 0.714344637831905
466 0.713114175703528
467 0.71211618450395
468 0.711144562941464
469 0.709905710846249
470 0.708793609786052
471 0.707858397244795
472 0.706693751505767
473 0.705803259171069
474 0.704698158263223
475 0.703854297261086
476 0.702822900207031
477 0.702001106286447
478 0.700996854088587
479 0.699842547694103
480 0.698883052601738
481 0.6979607483496
482 0.697041885276084
483 0.696173793409622
484 0.69503463217985
485 0.694084662162007
486 0.693155863466966
487 0.692198986997256
488 0.691376764204146
489 0.690282099061723
490 0.689720189511563
491 0.688781092740197
492 0.687862650043689
493 0.687001194165828
494 0.68597336404449
495 0.685081670549305
496 0.683995794911399
497 0.68329500517834
498 0.682266031776505
499 0.681452065358248
500 0.680793947206836
501 0.67999936210229
502 0.679080991569659
503 0.678203862811619
504 0.677224495583542
505 0.676503877441684
506 0.675656269071805
507 0.674903622174076
508 0.674256353299112
509 0.673440151540471
510 0.67252396422478
511 0.671602431234887
512 0.670863308340649
513 0.670005717620496
514 0.6690382160192
515 0.668231570051763
516 0.667254312536174
517 0.666248704513464
518 0.665376593249032
519 0.664708487590887
520 0.664025350576179
521 0.663249553530206
522 0.662354715598237
523 0.661466776131351
524 0.660780084878411
525 0.660012178224527
526 0.659062024389992
527 0.658236776446918
528 0.657424806929888
529 0.656609117810625
530 0.656015540391259
531 0.655245683807845
532 0.654594278060961
533 0.653762241948889
534 0.653133230634245
535 0.65232795565251
536 0.651627632634603
537 0.651029205708779
538 0.650338888637665
539 0.649466537160827
540 0.648855987154399
541 0.648044992683527
542 0.647193123379431
543 0.646305384313101
544 0.645555104121909
545 0.644776582177066
546 0.643784282700859
547 0.642926932595322
548 0.642191333761967
549 0.641394344480738
550 0.640339904117531
551 0.639578536361372
552 0.638899572058496
553 0.637997243576858
554 0.637092640518303
555 0.636304446521938
556 0.635463105736027
557 0.634851826344946
558 0.634083121219034
559 0.633193022568041
560 0.63238659739156
561 0.631510252864241
562 0.630780119696467
563 0.629962304019146
564 0.629212064846481
565 0.628406553011251
566 0.627773740821662
567 0.627103029323168
568 0.626216157416204
569 0.625446149744671
570 0.62467692076751
571 0.623959404271899
572 0.623163975805079
573 0.622571361777367
574 0.621940266307725
575 0.621014404082938
576 0.620264024523043
577 0.619516267258361
578 0.618803714003676
579 0.61819072242369
580 0.617559026435865
581 0.616758907448488
582 0.615892370920336
583 0.615335829823537
584 0.614567936920845
585 0.613922964734713
586 0.613454282694315
587 0.612628082035698
588 0.611936501170884
589 0.611245635978633
590 0.610726741836317
591 0.610042243779914
592 0.60951102588317
593 0.608850009595729
594 0.608359808547179
595 0.607535947576464
596 0.606970989849257
597 0.606294253683355
598 0.605768429333237
599 0.605197725691376
600 0.604534545779748
601 0.604002854432539
602 0.603285568766242
603 0.60249916919697
604 0.601794633629994
605 0.601077261553626
606 0.60045140133298
607 0.599852165491775
608 0.599233984329113
609 0.598470358671757
610 0.597841668927971
611 0.597281606727327
612 0.596527945362132
613 0.595960764437782
614 0.595461147796218
615 0.594862059190996
616 0.594322578252303
617 0.593610688156991
618 0.59293533371973
619 0.592434996621417
620 0.592007974192866
621 0.591435325713953
622 0.59086605899468
623 0.590303311110801
624 0.589659990714373
625 0.589135782881832
626 0.588566208859672
627 0.587914301115296
628 0.587331836996491
629 0.586702516098991
630 0.586127618828576
631 0.585671860551134
632 0.585158036080554
633 0.584524555849703
634 0.583860002973163
635 0.58339129313862
636 0.582887424427324
637 0.582192773459595
638 0.581661489099104
639 0.581017162795633
640 0.580726271239928
641 0.58014067311372
642 0.579461438806138
643 0.578963992580352
644 0.57839088468639
645 0.577663116556912
646 0.577100010319683
647 0.576420408314718
648 0.575883689425343
649 0.575293132564959
650 0.574686852661605
651 0.574174784233746
652 0.573627082282654
653 0.573058485563054
654 0.572426315307481
655 0.571991201312671
656 0.571273159597357
657 0.570705397879731
658 0.570036595762137
659 0.569568828057397
660 0.568822102021909
661 0.568309234682594
662 0.567725333589605
663 0.567132953299905
664 0.566581113689192
665 0.566044706899671
666 0.56547911397607
667 0.564901632747863
668 0.564291959119211
669 0.563742429075822
670 0.563198578413575
671 0.562571665873138
672 0.562065393031604
673 0.561497132273021
674 0.560915535726423
675 0.560373195003097
676 0.559898920288723
677 0.559423555941699
678 0.558723728873759
679 0.558177940605194
680 0.557527249828042
681 0.556881134720179
682 0.556202118354029
683 0.555672944441776
684 0.555165400148381
685 0.554502701298611
686 0.553882239421793
687 0.553287853554268
688 0.552708500911845
689 0.551930238559589
690 0.551305341382344
691 0.550720899340665
692 0.550039199047484
693 0.5493891830501
694 0.548688643089202
695 0.548031492001947
696 0.547309895862607
697 0.546609936104083
698 0.546053980032399
699 0.545300741201627
700 0.544674341731222
701 0.544136512162727
702 0.543491799830111
703 0.542828890730231
704 0.542112715388248
705 0.541461382162609
706 0.540718394346093
707 0.539909950259768
708 0.539353404528331
709 0.538634926359429
710 0.537923455616571
711 0.53718304128477
712 0.536529737601367
713 0.535892984804421
714 0.535257728748591
715 0.53463377273857
716 0.533833506197229
717 0.533150214536628
718 0.532415123837147
719 0.531808633850299
720 0.531181474868321
721 0.530483243674373
722 0.529904573342939
723 0.529395009496604
724 0.528863932256406
725 0.528274191793741
726 0.527737637467208
727 0.527070507872942
728 0.526468072780012
729 0.52586698538938
730 0.525364411118084
731 0.52476437375604
732 0.524151683159629
733 0.523561852451089
734 0.52289410527936
735 0.52219237615492
736 0.521561706106352
737 0.520916911156826
738 0.520245115865341
739 0.519565222932346
740 0.519057424972815
741 0.518560277193055
742 0.518027052206282
743 0.517387945953778
744 0.516671145777221
745 0.516010697701994
746 0.515316980947466
747 0.514555281940236
748 0.513840908689076
749 0.513266557162999
750 0.512552093816703
751 0.511823272381991
752 0.511157954487136
753 0.510503528303388
754 0.509829728718814
755 0.508996661716358
756 0.508352907990492
757 0.507552142860409
758 0.506828226642083
759 0.505962424978266
760 0.505158441187779
761 0.504391063798505
762 0.503704798078003
763 0.503041641953015
764 0.502266988288105
765 0.501543429779812
766 0.500823888715215
767 0.500113634895374
768 0.499330549168328
769 0.498577968279438
770 0.497670890384991
771 0.496995118561804
772 0.496273670446773
773 0.495540644029516
774 0.494839638105705
775 0.49411387841511
776 0.493316041083234
777 0.492596538307109
778 0.4919420687499
779 0.491161371568554
780 0.490454157389128
781 0.489734269394812
782 0.489028622126729
783 0.488293290303655
784 0.487718961470544
785 0.48699489747094
786 0.486426862802784
787 0.485649323372786
788 0.48502222457019
789 0.484483857799829
790 0.483878963133306
791 0.483160497421244
792 0.482595111538211
793 0.481820143403649
794 0.481200283281126
795 0.480470998823027
796 0.479737572570214
797 0.47900997107336
798 0.478260896808424
799 0.477622594567338
800 0.476788233282963
801 0.476097693383462
802 0.475456868411142
803 0.47476838333093
804 0.473968376320975
805 0.473245953241207
806 0.47262335423575
807 0.471946262348108
808 0.471228236774394
809 0.470487412608542
810 0.469843722155711
811 0.469160620225497
812 0.468341251687196
813 0.467799657977283
814 0.467061161025431
815 0.466453259431549
816 0.465598639031216
817 0.464947718597547
818 0.464253406029003
819 0.463636109330645
820 0.462986368703654
821 0.46236782977917
822 0.461613009569369
823 0.460983452341785
824 0.460404978459837
825 0.459769372791899
826 0.459214127757751
827 0.458598130250471
828 0.457935470943034
829 0.457350476027233
830 0.456676883525272
831 0.455937928772312
832 0.455371047035121
833 0.454693060178284
834 0.453993248714035
835 0.453297946124553
836 0.452719202051052
837 0.452129349863051
838 0.451505165991084
839 0.450918732299909
840 0.45027935385137
841 0.449621392251141
842 0.448924479431336
843 0.448322817780947
844 0.447699119297225
845 0.447069354077762
846 0.446358009845774
847 0.445749082670981
848 0.445136327844513
849 0.444427975552049
850 0.443871307453416
851 0.443235514586366
852 0.442758977816567
853 0.442185085015707
854 0.441533654791021
855 0.440836362162393
856 0.440351006132969
857 0.439837257199891
858 0.439308302771224
859 0.438790889722482
860 0.438398235800337
861 0.437784025545746
862 0.437341661065116
863 0.436904199439935
864 0.436429321564438
865 0.436110897063677
866 0.435627708578464
867 0.435232372995169
868 0.434802506281117
869 0.434371168199157
870 0.433890836076771
871 0.433328260347814
872 0.432839776420231
873 0.432442621378515
874 0.431937361628764
875 0.431406977976724
876 0.430926071941744
877 0.430458371744777
878 0.430020686735113
879 0.429449523305298
880 0.428977597663485
881 0.428548958208533
882 0.428236589946331
883 0.427731776788613
884 0.427214538450841
885 0.426780147677092
886 0.426294920586931
887 0.425880452958427
888 0.425269028254709
889 0.424808545925169
890 0.424483400199042
891 0.42405210406643
892 0.42376930100699
893 0.423345589983181
894 0.422953665558667
895 0.422511628435584
896 0.422153962477949
897 0.421776741062916
898 0.421434411564901
899 0.42105716781047
900 0.420779018337303
901 0.42033492542802
902 0.419957179890755
903 0.419656182162972
904 0.419242646294356
905 0.418899852375609
906 0.418593077660114
907 0.418308330575484
908 0.417910249970426
909 0.417586172557986
910 0.417242422467965
911 0.416892290899708
912 0.416594039989139
913 0.416247387372248
914 0.415973443824116
915 0.415674819345975
916 0.415302314740645
917 0.41496415742712
918 0.41464559755563
919 0.414295212817848
920 0.413953612959382
921 0.413473358402684
922 0.413064258197053
923 0.412860626402589
924 0.41254056774574
925 0.412163912593502
926 0.411825868012394
927 0.411509733675749
928 0.411178410728235
929 0.410851353352207
930 0.410538796919464
931 0.410306859819658
932 0.410024258246001
933 0.409727070057289
934 0.409383253685383
935 0.40904635889111
936 0.408771136454242
937 0.408598527832806
938 0.408265546142928
939 0.408058580634502
940 0.407946446868714
941 0.407725928189084
942 0.407458025818444
943 0.407304883431842
944 0.407120461024554
945 0.406965822036801
946 0.40653702212696
947 0.406209016830317
948 0.40598135445369
949 0.405768053921601
950 0.405514149532116
951 0.405322960632892
952 0.405024831660029
953 0.404781940081771
954 0.404581335142739
955 0.404358581136427
956 0.404101826306026
957 0.40387595604483
958 0.403595021432006
959 0.403410966690563
960 0.40316532614958
961 0.403026909148902
962 0.4028877754479
963 0.402694699640485
964 0.402570425478174
965 0.402340587756183
966 0.402244416130574
967 0.402025392201674
968 0.401799256202353
969 0.401556660274149
970 0.401460184744212
971 0.401255150052417
972 0.401073538433008
973 0.400955634689921
974 0.400818676187164
975 0.400679356453332
976 0.400478540584551
977 0.400323937489206
978 0.400276565331974
979 0.400166152864405
980 0.400080664166678
981 0.399984757751078
982 0.399884798798861
983 0.399801006009163
984 0.399743667848858
985 0.399670078723339
986 0.399391725470554
987 0.39930104262425
988 0.399196062049752
989 0.399003392434255
990 0.398925686223825
991 0.398901240945555
992 0.39881375155842
993 0.398716782271089
994 0.398674702227799
995 0.398639291104561
996 0.398529057455284
997 0.398515761731474
998 0.398486001797722
999 0.398413149663318
1000 0.398378920693837
};
\addlegendentry{random sampling}
\end{axis}


